Distributed creation of Machine learning agents for Blockchain analysis

Creating efficient deep neural networks involves repetitive manual optimization of the topology and the hyperparameters. This human intervention significantly inhibits the process. Recent publications propose various Neural Architecture Search (NAS) algorithms that automate this work. We have applied a customized NAS algorithm with network morphism and Bayesian optimization to the problem of cryptocurrency predictions, where it achieved results on par with our best manually designed models. This is consistent with the findings of other teams, while several known experiments suggest that given enough computing power, NAS algorithms can surpass state-of-the-art neural network models designed by humans. In this paper, we propose a blockchain network protocol that incentivises independent computing nodes to run NAS algorithms and compete in finding better neural network models for a particular task. If implemented, such network can be an autonomous and self-improving source of machine learning models, significantly boosting and democratizing the access to AI capabilities for many industries.

==> content/common_content.tex <==
\section{Background}
\label{background}

The following subsections describe basic blockchain and deep learning concepts.

\subsection{Blockchain and Ethereum}

%is this really needed?
Satoshi Nakamoto's introduction of Bitcoin in November 2008 \cite{bitcoin-paper} has often been hailed as a radical development in money and currency as it's the first example of a digital asset which simultaneously has no backing or ``intrinsic value'' and no centralized issuer or controller. Another arguably more important part of the Bitcoin experiment is the underlying blockchain technology as a tool of distributed consensus. The most important aspect of such technology is the absence of an intermediary (centralized server, bank, company, etc.) between the originator and the recipient, as any changes to the data on this chain are made by consensus among all members of a decentralized network. Thus, avoiding the need to trust third parties. The blockchain can be thought of as a distributed public database with records for each transaction in history. All cryptoasset operations and activity are contained within the blockchain transaction data.

The Ethereum project ($ETH$) is a newer implementation \cite{yellowpaper}, based on the blockchain technology. In addition to the transaction record keeping functionality, Ethereum provides a mechanism for executing program logic on each transaction, thus enabling a much wider variety of use cases of the blockchain technology. Some of which include financial transactions, secure voting, autonomous organizations, company management, freedom of speech networks, online games, crowdfunding, speculation, making it one of the more noisy and difficult to predict blockchains.

\subsection{Autonomous decentralized applications}

The intent of Ethereum is to create an alternative protocol for building autonomous decentralized applications. Because of the blockchain consensus, no one has control over the code execution or storage of these applications. A decentralized application can not be modified outside of the constraints of its logic. Because such an immutable application resembles contractual relations, autonomous decentralized applications are often referred to as ``crypto contracts'', ``smart contracts'' or simply contracts.

\subsection{Transactions and traces}

Every block in the chain is a package of transactions. Every transaction denotes a transfer of value and/or an execution of a smart contract.

Transactions only contain information about the initial (outside) call. For example, if a contract receives funds from $x$ and forwards them to $y$, the transaction will only indicate that the contract received the funds. The transfers the contract additionally makes are known as internal calls. To gather information about them, the initial transaction needs to be replayed in order to observe the derivation from it. Transfers and contract activities collected using this method are called $traces$.

\subsection{Factors for digital asset value change}

In basic economics, the correlation between supply and demand \cite{supply_demand} determines the price of an asset. Higher demand or lower supply relates to higher price.


Because of small market capitalization, digital currencies are unstable and volatile. Based on our observations of Ethereum, we have identified multiple factors as having a significant influence on the supply and demand of the currency. Most of them can be traced by analyzing the blockchain data in depth.

\subsubsection{Speculative investment}

%PLEASECITATIONNEEDED

Speculative investment is the action of buying and holding a certain asset, speculating that its value will rise in the future. This hampers Ethereum's already low supply and results in artificial price increases.

%In our research, we investigate methods that track the influence of this behaviour to the asset's price.

\subsubsection{Initial Coin Offerings}

Intial Coin Offerings (ICOs) \cite{ico} are share resemblance to Initial Public Offerings, but are implemented using smart contracts and therefore do not bear any of the legal protections that regular investments provide.

During 2017, the total cumulative ICO funding has increased by more than $80$ times \cite{ico-funding}. Ethereum's smart contract framework has become the most targeted platform for ICO fundraising. This is believed to have been a major reason for Ethereum's rise during June 2017.

%We track ICO activities on the blockchain in attempts to observe their impact on value changes.

\subsubsection{Altcoin interference}
\label{altcoin-interference}

After Bitcoin, hundreds of other cryptocurrencies have emerged. Despite the fact that they are completely unrelated and independent from each other, major events in one cryptocurrency can cause unexpected fluctuations in others. For example, major ICO events in Ethereum have caused surges in numerous other currencies, like Litecoin \cite{litecoin}. 

%Currently our prediction models do not take into account the altcoin interference. Our goal is in a further research to include data from other blockchains into our datasets.


%we don't track any such data.
%Should we mention the first sentence? Is it not obvious that it leads to a research ?
%The interference of other alternative coins to Ethereum leads to a whole research topic on its own. We have plans to include historical data and events from other currencies to improve our predictions.

\subsubsection{Media influence}
\label{media-influence}

Crypto market's value can also be easily influenced by media publications. A prime example of this is a case of widespread hoax about an incident with Ethereum's founder Vitalik Buterin \cite{vitalik-death}. This led to temporary plummet and loss of 4\$ billion from Ethereum's market capitalization.

Currently our prediction models do not take into account the media influence. Our goal is in a further research to perform deep-learning based sentiment analysis on news and social media sources related to cryptocurrencies.

%we don't get such data yet, is that a problem?
%In a further research, we will experiment with cases where we track the news stories about Ethereum and similar cryptocurrencies via sentiment analysis.

%\subsubsection{Attacks and thefts}

%Ethereum's smart contract framework is anything but flawless. The immutability and publicity of smart contracts have placed many in concerns that a published contract with flawed code can be attacked and exploited. There have been countless moments of Ethereum's history where similar events have occured. The first major disaster was ``The DAO'' hack, where a hacker stole 50M\$ worth of ETH due to a vulnerability in the contract \cite{dao}. Very recent, and unfortunately much more catastrophic, are two attacks on parity's multi-signature wallet. The first attack was due to a security vulnerability in the contract which resulted in 30M\$ worth of ETH being stolen \cite{parity1}. The second attack happened following the fix of the initial vulnerability, which opened another vulnerability in the process. The result was 300M\$ worth of ETH being completely frozen and unusable, likely forever \cite{parity2}.

%Other than smart contract related attacks, the usual cryptocurrency thefts still stand. Cases where money are sent to the wrong address, someone reveals the private key of an account or simply fools people into sending him ETH for a promise are a common occurrence. There are no consumer protections and no real way to get money returned, if their current owner doesn't want to.

%We will track closely smart contract activity, as well as unusual transfers of tokens to increase our prediction accuracy.



\subsection{Use of Deep Learning in asset value predictions}
Deep Learning \cite{deep_learning} allows for the discovery of patterns in a large dataset. Such a set consists of called dataset samples (forming input-output pairs, such as summarized blockchain activity and the future price). The inputs pass through multiple layers (which perform data transformations with free parameters) and leave as an output. The free parameters have to be set (trained, learned) on known input-output pairs.

Long Short-Term Memory (LSTM) \cite{LSTM} and Convolutional (CNN) \cite{cnn} networks are types of DL networks, which are well known for their performance in time series and image analysis respectively.

\subsubsection{Normalization}
\label{normalization_bg}

%a single value cannot have zero mean and equal variance
Every value in a dataset needs to be normalized (scaled, fit), because of the numerical instability of large computer floating point operations. The general objective for a normalized series is to consist of small numbers of zero mean and equal variance. We use the following normalization algorithms depending on the situation:

$$basic_i = \frac{x_i - min(x)}{(max(x) - min(x))}$$

This basic min-max scale is used to map independent sequences with the same sign to the interval $\in [0; 1]$.

$$around\_zero_i = \frac{x_i + max(\lvert max(x) \rvert, \lvert min(x) \rvert)}{2*max(\lvert max(x) \rvert, \lvert min(x) \rvert)}$$

Similar to $basic$, but maps positive and negative inputs to $(0.5; 1]$ and $[0; 0.5)$ respectively. This scale is used with sequences of varying sign.

%do I need to specify what is std?
$$image_i = (x_i - \frac{1}{n}\sum_{t=1}^{n}x_t) * \frac{1}{std(x)}$$

An an algorithm which produces unbounded time series of zero mean and equal variance. It is used with image-line sequences.
%$$local_i = \frac{win_i}{win_0} - 1$$

%Local normalization based on the first element of a window of values. As it does not depend on the whole sequence, it can normalize future values without issue.
%we don't use sigmoid. Remove it?
%$$sigmoid_i = \frac{1}{1 + \exp(-arr_i)}$$

%Non-linear normalization function that provides consistent normalization no matter the sequence. We recommend this to be used with relatively small values, as normalizing large enough values results in a practically indistinguishable difference in the output value.

\subsubsection{Error measures}
\label{measures}

The following measurement factors are often used to evaluate the performance of predictive DL:

$$
\hspace{2ex}sign = \frac{t}{t+f};
\hspace{2ex}err(t) = out_t - true_t;
\hspace{2ex}null(t) = 0.5 - true_t
$$

$$MSE = \displaystyle\frac{1}{n}\sum_{t=1}^{n}err(t)^2;
\hspace{0.5ex} RMSE = \sqrt{\displaystyle\frac{1}{n}\sum_{t=1}^{n}err(t)^2};
\hspace{0.5ex}R^2 = 1-\displaystyle\frac{\sum_{t=1}^{n}err(t)^2}{\sum_{t=1}^{n}null(t)^2}
$$

%custom = \displaystyle\frac{1}{n}\sum_{t=1}^{n}\frac{\lvert err_t \rvert}{min(pred_t, true_t)};

Where $out$ and $true$ are lists of outputs and expected outputs respectively. If the outputs are binary, then the amount of correctly and incorrectly predicted flags is $t$ and $f$ respectively.

The metrics $R^2$ and $sign$ measure accuracy $\in [0, 1]$, this the aim is to maximize them. In $R^2$ the performance of the model is compared to that of a model always returning the same value. $MSE$ and $RMSE$ are measures of error which have to be minimized.
%In efforts to observe our network's performance from different angles, we have created our own error function, called $custom$.

Traditionally, $MSE$ is used as the loss function during training. The rest are used for performance analysis.

\section{Raw data}
\label{data-sources}

The first kind of data gathered is historical market tick data, which is aggregated from multiple exchanges to achieve a less biased view of the financial state. The frequency (size of each tick) is one hour. Every tick consists of the $open$, $close$, $low$, and $high$ prices, as well as the trade volume to and from the currency for that period. 

The second kind of data is from the Ethereum blockchain. It grows every day \cite{blockchain-size} and includes hundreds of gigabytes worth of transactions, cryptocontract executions, and blockchain events for every moment its existence. For each block in the chain, the following data points are extracted: creation timestamp, number (chain index), miner (block creator), list of confirmed transactions, size in bytes, creation difficulty, and computational resources used (Gas limit and Gas used). The following is stored for each transaction in a block: address of the initiator and receiver, transferred value, used resource units (Gas), and amount paid per resource unit (Gas price). The same kind of information is also collected for internal contract activity by calculating transaction traces.

The total size of the gathered raw blockchain features is around 500GB, containing $5,300,000$ blocks with a total of $194,000,000$ transactions and close to a billion traces. It took 30 consecutive days to download and another 14 to process, filter, format, and save the data to a database.

Both the market and blockchain data are collected for the interval from 8-08-2015 to present.

\section{Generation of data properties}
\label{property-generation}

In order to create a blockchain-based dataset, we first need to extract the most valuable information from the raw blockchain data by performing different feature extraction algorithms. A feature (also called property) is calculated once for each market tick in the historical data in order to form a time series.

We are extracting a set of properties defined in Table \ref{properties}. They are created and selected based on their importance and significance to the prediction problem. A property name with suffix ``$\_rel$'' denotes that its values have been converted to relative ones. An example for a property is seen in Figure \ref{propertyGasUsed}.

\begin{table}[h]
\centering
\caption{\label{properties}List and description of the properties compiled from the raw data.}
\begin{tabular}{lp{5.5cm}}
Property & Description \\
\hline
openPrice & The value of ETH at the start of the tick \\
closePrice & The value of ETH at the end of the tick \\
stickPrice & $openPrice - closePrice$ \\
volumeTo & Exchange volume to that cryptocurrency \\
volumeFrom from & Exchange volume from that cryptocurrency \\
transactionCount & Amount of transactions  \\
dappOperations & Amount of transactions to crypto contracts \\
blockSize & The average size of a block in bytes \\
difficulty & The average difficulty for block mining \\
uniqueAccounts & Number of accounts in existence \\
gasLimit & Average limit on computational resource use \\
gasPrice & Average price per gas unit \\
gasUsed & Average amount of gas used \\
networkHashrate & Combined hashrate of every miner in the network \\
ETHSupply & Total amount of Ether in circulation \\
pendingTx & How many transactions per minute are pending for inclusion in the next block \\
blockchainGrowth & Growth of the blockchain size in gigabytes \\
\end{tabular}
\end{table}

%may be too tiny.
\begin{figure}[h]
\centering\includegraphics[width=\graphwidth]{assets/property_graph}\\
\centering\includegraphics[width=\graphwidth]{assets/property_graph_rel}
\caption{The absolute (up) and relative (down) values of property $gasUsed$ over time. We can observe how major events have influenced the usage of the Ethereum network over time.}
\label{propertyGasUsed}
\end{figure}

The following subsections explain more advanced concepts in calculating properties.

%removing since it isn't used in our experiments
\texcomment{
\subsection{Technical indicators}
Our property values include significant amount of statistical noise which can hamper the training process. We smoothen all of our property values through a set of statistical functions, which are successfully applied in numerous of prediction strategies on the stock market. The functions include Simple Moving Average ($SMA$) and Exponential Moving Average ($EMA$). All of our functions use 10 tick intervals. Property names with suffixes ``$\_sma$'' and ``$\_ema$'' denote that the property values are modified by the respective function. 
}

\subsection{Distributions}

Other than extracting singular value properties like the discussed so far, we are also investigating ways to extract more valuable information from the blockchain by tracking the activity of the crypto accounts in higher detail. This is achieved by creating account distributions- 2D matrices that visualize account activity based on multiple account features. These distributions contain spatial value, which Convolutional networks can take advantage of. 

Let us introduce some common definitions: $scl$ as an array of scale functions, $feat$ as an array of functions that return an account feature, and $mx$ as an array of constants.

Possible values for $scl_i$ include $\log_2$ and $\log_{1.2}$. Possible account features ($feat_i$) are defined in Table \ref{account_feature_table}.

\begin{table}[h]
\centering
\caption{\label{account_feature_table}The possible account feature functions.}
\begin{tabular}{lp{6cm}}
Feature & Description \\\hline
balance & Account balance, measured in $wei$ ($10^{18}$ $wei$ = 1 $ETH$). \\
lastSeen & Amount of seconds since the account's last participation in a transaction. \\
volumeIn & Amount of received value in the last tick, in $wei$. \\
volumeOut & Amount of sent value in the last tick, in $wei$. \\
transactionN & Amount of transactions where the account as either a receiver or a sender.\\
ERC20 & Amount of ERC20 token operations in the last tick (Ethereum contracts only) \\
\end{tabular}
\end{table}

\subsection{Account balance distribution}
\label{account_balance_distribution}

This distribution visualizes summarized recent account activity in terms of the exchanged volume and amount of transactions, distributed based on balance groups.

\vspace{3em} %tmp

Let us define $scl_0 = \log_2 \; mx_0=10^{26} \; feat_0=volumeIn \; feat_1=volumeOut \; feat_2=transactionN \; groupN = \lfloor\ scl_0(mx_0)\rfloor \; featN=3 $, $S$ as the accounts that have participated in a transaction in the current market tick, and $distribution$ as a matrix of shape $(featN, groupN)$.

For $acc \in S$:

\hspace{3em} $gr = \min(\lfloor scl_0(balance(acc))\rfloor, groupN-1)$

\hspace{3em} For $x \in [0, featN)$:

\hspace{6em} $distribution_{x, gr} \; += feat_x(acc)$

$distribution = scl_0(distribution)$

The final operation is to scale the large values of volumeIn and volumeOut.

Figure \ref{account_balance_graph} contains an example of $2$ such distributions.

\begin{figure}[h]
\centering\includegraphics[width=\graphwidth]{assets/distributions/accountBalanceDistribution_log1_2}\\
\centering\includegraphics[width=\graphwidth]{assets/distributions/accountBalanceDistribution_log2}
\caption{Examples with $scl_0=\log_{1.2}$ (up) and $scl_0=\log_{2}$ (down). We observe how the summarized account trade activity changes in the different balance groups.}
\label{account_balance_graph}
\end{figure}

\subsection{Account number distributions}
\label{account_number_distribution}

These multivariate distributions represent how the accounts are clustered based on 2 of their account features.

The process of creating an account number distribution is described as follows:
\vspace{1em}

Repeat for $x = 1$ and $x = 2$:

\hspace{3em} $groupN_{x} = \lfloor scl_{x}(mx_{x})\rfloor$

For $acc \in S$, where $S$ is a chosen subset of (or all) accounts, do:

\hspace{3em} Repeat for $x = 1$ and $x = 2$:

\hspace{6em} $group_{x} = \min(\lfloor scl_{x}(feat_{x}(acc))\rfloor, groupN_{x}-1)$

\hspace{3em} $distribution[group_1, \; group_2] \; += 1$

Finally, for every value, do:

\hspace{3em} $distribution = \log_2(distribution)$

The final $\log_2$ scaling is to mitigate the uneven distribution of accounts. The possible options for the $feat$ functions are defined in Table \ref{account_feature_table}. Some configurations of distributions are presented in Table \ref{account_number_table} and are later referred to in the experiments.

\begin{table}[h]
\centering
\caption{\label{account_number_table}The configurations for account number distributions.}
\setlength\tabcolsep{1.5pt} % TEMPORARY FIX
\begin{tabular}{lrrrrrrrp{5cm}}
$N$ & $S$ & $feat_1$ & $feat_2$ & $scl_1$ & $scl_2$ & $mx_1$ & $mx_2$ \\\hline
1 & all & balance & lastSeen & $\log_{1.2}(\lfloor x / 10^{17} \rfloor)$ & $\log_{1.2}$ & $10^{7}$ & $20736e3$ \\
2 & contracts & balance & lastSeen & $\log_{1.2}(\lfloor x / 10^{17} \rfloor)$ & $\log_{1.2}$ & $10^{7}$ & $20736e3$ \\
3 & contracts & volumeIn & ERC20 &  $\log_{2}(\lfloor x / 10^{17} \rfloor)$ & $\log_{2}$ & $10^{7}$ & $262144$ \\
\end{tabular}
\caption*{The balances and transfers, measured in wei, are scaled to larger units ($10^{17}$ $wei$ = $0.1$ $eth$) to reduce noise.}
\end{table}

Consequently, we refer to the distribution configurations as follows: balanceLastSeenDistribution (N=1), contractBalanceLastSeenDistribution (N=2), and contractVolumeInERC20Distribution (N=3). Example distributions are visualized in Figure \ref{account_number_example}.

\begin{figure}[h]
\centering\includegraphics[width=0.8\graphwidth]{assets/distributions/balanceLastSeenDistribution_log1_2}\\
\centering\includegraphics[width=0.7\graphwidth]{assets/distributions/contractVolumeInERC20Distribution_log2_v2_stateless}
\caption{
\textbf{balanceLastSeenDistribution (up)}: we observe the difference in activity of the most active accounts (left) and richest accounts (down). The empty lines are seen because $\lfloor\log_{1.2}(x)\rfloor \notin \{1, 2, 4, 5\}$ for all $x$.
\if\showlinks1
User behavior and major market movements are more effectively seen in a time-lapse video of the distribution values (\href{https://youtu.be/Dwwnxn1j6AQ}{https://youtu.be/Dwwnxn1j6AQ}).
\fi
\textbf{contractVolumeInERC20Distribution (down)}: we observe the different proportions of a crypto contract being used ($X$) and the amount of funds received from it ($Y$).
}
\label{account_number_example}
\end{figure}

\section{Generation of a dataset}

A dataset is a set of samples, containing inputs (normalized property data) and expected outputs (prediction target). The concepts and methodologies behind dataset generation are defined in the following subsections.

\label{dataset-generation}

\subsection{Prediction target}
%not sure if 51% attacks should be mentioned
The prediction target is the future value a chosen target property. Predictions are for the duration of one market tick. Examples of a prediction target include relative price fluctuations, amount of new accounts, trade volume, transaction count and network clogging (a serious issue in the light of recent events \cite{blockchain-clogging}).
%or possibly attempts of 51\% attacks \cite{51attack}.

Our experiments will be mainly focused on predicting price movements and new accounts.

\subsection{Normalization}
\label{normalization}

Every property in a dataset is a different time series and is normalized separately with a chosen algorithm (among those defined in Secion \ref{normalization_bg}). A method to automatically determine the algorithm for a given property is called $prop$, which uses $basic$ scale if the property values are absolute and $around\_zero$ scale otherwise.

Most of the algorithms scale on the basis of $\min$ and $\max$ bounds, hence future values may not fit that initial scale. The problem is mitigated if the normalized values are relative, which has also resulted in lower overfit and higher prediction accuracy in our experiments.
%the below technique is not used
%We also use a technique called normalization space overprovisioning, which increases the initial $\min$ and $\max$ values by a given percentage so that future values are more likely to fit.
%The problem of future values can be solved completely by using $local$ normalization, but that is not the best algorithm in all cases.
%All of the aforementioned methods to deal with the problem can be used in conjunction with each other.

\subsection{Dataset models}
\label{dataset-models}
The dataset samples (input-output pairs) are created using a sliding window with a size of $wn$ and step increments of $1$ over a chosen set of normalized property values. Let us define a property's values as $prop_y$, where $y < propN$, a specific value in a property time series as $prop_{y,x}$, and $prop_{t}$ as the prediction target.

%$step=0$

For $x \in [0, wn-1]$, do:

\hspace{3em} For $y \in [0, propN-1]$, do:

\hspace{6em} $win_{x,y} = prop_{y,x+step}$

\hspace{0em} $tar = prop_{t, wn+step}$

Where $win$ is the window (unstructured dataset input), $tar$ is the expected output, and $step$ is incremented for each window.

In order to combine multiple normalized properties in a single dataset, we need the following models that define how their values are arranged in N-dimensional space.

\subsubsection{Matrix model}

Based on the LSTM network's 2D input shape, the matrix model defines one dataset sample as being the same as its corresponding $win$, without modifying its structure in any way.

Table \ref{matrix_model_table} visualizes the structure of a dataset sample.

\begin{table}[h]
\centering
\caption{\label{matrix_model_table}Example of a matrix model dataset sample.}
\begin{tabular}{lrrr}
Property & Value $0$ & Value $1$ & ... Value $wn-1$ \\\hline
Close value & 349\$ & 358\$ \\
Number of TXs & 2876 & 1583 \\
Operations with Contracts & 459 & 508 \\
\end{tabular}
\end{table}

\subsubsection{Stacked layers model}
\label{stacked-model}

%\begin{wrapfigure}{R}{0.5\graphwidth}
\begin{figure}
%\centering\includegraphics[width=\linewidth]{assets/stacked_model}
\centering\includegraphics[width=0.5\graphwidth]{assets/stacked_model}
\caption{Visualized sample of the stacked layers model, where $wn=3$ and the chosen properties consist of balanceLastSeenDistribution.}
\label{stacked_model_example}
\vspace{-0pt} %workaround, because wrapfigure hates the float package
%\end{wrapfigure}
\end{figure}

A given set of property values (a column in $win$) has shape $(v_1, v_2, wn)$, where $v_1 = 1$ and $v_2 = 1$ for all properties but the distributions (discussed in Sections \ref{account_balance_distribution} and \ref{account_number_distribution}); these properties with windowed values of 3D shape can't be modeled by a matrix. The stacked layers model is a 3D structure that matches input shape for the Convolutional Neural Network and allows modeling of 3D shaped property windows, preserving their spatial value. 

The model defines a 3D matrix $mat$ of shape $(values_1, values_2, wn)$. A dataset sample $mat$ is created as follows. For every set of windowed property values $vals$:

$$mat_{s_1 + (0 \; to \; v_1), s_2 + (0 \; to  \; v_2), 0 \; to \; wn} = vals_{0 \; to \; v_1, 0 \; to \; v_2, 0 \; to \; wn}$$

Where $s_1$ and $s_2$ are set to the smallest integers where no values of other previously assigned properties are overridden. A visualized sample produced this model is seen in Figure \ref{stacked_model_example}.

\vspace{1pt} %to move the title of the next section to the next page


==> content/content_bg.tex <==
\section{Въведение} 

Криптовалутите, децентрализираните нови начини за обмен на стойност, набират голям интерес напоследък с появата на Bitcoin, Ethereum и стотици други криптоактиви с обща пазарна оценка от над \$500 милиарда. За разлика от традиционните пазари, където всички данни за пазара и самата търговия са централизирани и контролирани от организации, криптоактивите са публични и децентрализирани. Този нов вид данни в блокчейна предоставя уникална възможност за разработване на по-стабилни прогнозиращи системи. 

%say that blockchain is volatile and price data just won't cut it - comparison with world economical crisis 
Повечето прогнози за стойността на валути се основават предимно на предишни движения на цената. Тези стратегии обаче се представят много слабо при малките и нестабилни пазари на криптовалутите. За да преодолеем това, в допълнение към пазарни данни, ние можем да анализираме публичните данни в блокчейна в усилия да прогнозираме бъдещи факти. 

%something about the framework? 
%state how much is lost by volatility 

Проучвания в прогнози за стойността на криптоактиви са били публикувани досега - експерименти от екип на университета Станфорд \cite{stanford-predictions} на тема Bitcoin ценови прогнози е са били публикувани през 2014 г. Те събират данни от блокчейна на Bitcoin, но се съсредоточават върху основни мерки, като броя на последните транзатции, без да влизат в дълбочина, примерно с дистрибуции на балансите на акаунтите. Повечето грешки в техните прогнози са грешни положителни сигнали, което сигнализира за ниска генерализация на техните невронни модели. Нужните подробности за повтаряне на техните резултати не са разкрити в описанието. Още два нови проекта, достъпни в Github, също изследват Bitcoin прогнози \cite{bitpredict} \cite{deep-learning-bitcoin}, но и двата се фокусират предимно върху исторически пазарни данни и не разкриват своята обработка на данни или използваните невронните архитектури. 

\subsection{Цели на проекта} 
%'should be' or 'is' 
Нашата цел е да проучим как съвременните техники за дълбоко машинно самообучение могат да бъдат приложени при прогнози на бъдещи стойности на криптоактиви. По-конкретно, ние се интересуваме дали можем да използваме множеството данни в блокчейна за повишаване на точността на нашите прогнози. 

Целта ни е да създадем гъвкава и отворена рамка за прогнози на криптовалути. Рамката позволява събирането на блокчейн и пазарни данни и осигурява начин за бърза имплементация на алгоритми за обработка на данни и за извличане на свойства. Извлечените характеристики (или свойства) са компилирани в датасет, използвайки определени пространствен модели. Невронните архитектури са изградени, тренирани, оценени и сравнени. Целта на прогнозите може да бъде всяка характеристика на крипто-валутата, а не само движенията на цената. 

Стигнахме до извода, че Ethereum ($ETH$) \cite{yellowpaper} вероятно е най-предизвикателната среда за прогнози, поради голямата си и гъвкава потребителска база. Приложенията на технологията включват пазарни транзакции, сигурно гласуване, автономни организации, управление на компании, мрежи за свобода на словото, онлайн игри, публично финансиране, спекулации и др. Тази стохастична среда най-добре ще покаже истинската точност на нашите стратегии за прогнози, които после могат да бъдат мигрирани до по-стабилни блокчейни, като Bitcoin. 

За да създаваме имплементация на нашата рамка за Ethereum е нужно да изучим историята на мрежата, потребителите и поведението им, да посочим факторите за нестабилност и да предложим и тестваме стратегии за преодоляване на затрудненията. Ние ще се фокусираме предимно, но не изцяло, върху ценови прогнози. Промените в стойността обикновено са последвани от съответни промени в други характеристики на блокчейна. 

\subsection{Блокчейн и Ethereum} 


%is this really needed? 
Представянето на Bitcoin от Satoshi Nakamoto през ноември 2008 г. \cite{bitcoin-paper} често приветствано като радикална промяна в парите и валутата, като първият пример за цифров актив, който едновременно е без ``същинска стойност'' и няма централизиран източник или регулатор. Друга, спорно по-важна, част от Bitcoin експеримента обаче е основаната блокчейн технология, като средство за разпределен консенсус. Най-важният аспект на тази технология е липсата на посредник (централизиран сървър, банка, компания и т.н.) между инициатора и получателя, понеже всички промени в данните са извършени чрез консенсус между всички членове на децентрализираната мрежа. По този начин се избягва нуждата от доверие към трети страни. 

Ethereum ($ETH$) е скорошна имплементация \cite{yellowpaper} на блокчейн технологията. В допълнение към функиалността за съхранение на транзакции, Ethereum предоставя и механизъм за изпълнение на програмна логика, като по този начин дава възможност за много по-голямо разнообразие от приложения на блокчейн технологията.

\subsection{Автономни децентрализирани приложения} 

Целта на Ethereum е да създаде алтернативен протокол за изграждане на автономни децентрализирани приложения. Поради консенсуса на блокчейна, никой индивидуално няма контрол върху изпълнението или съхранението на тези приложения. Децентрализирано приложение не може да бъде спряно, изтрито или атакувано по някакъв начин, освен ако логиката му не го позволява. Тази функционалност наподобява договорни отношения и затова тези приложения са често наричани ``криптодоговори'' или просто договори. 

\subsection{Фактори за промяна на стойността на активи} 

В основите на икономиката, съотношението между търсене и предлагане \cite{supply_demand} определя цената на даден актив. Високо търсене или ниско предлагане е свързано с по-висока цена.

Поради ниска пазарна капитализация, дори сравнително малките промени в търсенето и предлагането на цифровите валути водят до съществени промени в цената, което ги прави нестабилни и непредсказуеми. В следствие на нашите наблюдения при Ethereum, ние установихме, че следните фактори оказват значително влияние върху търсенето и предлагането на валутата. 

\subsubsection{Спекулативно инвестиране} 

%PLEASECITATIONNEEDED 

Спекулативното инвестиране е купуване и задържане на даден актив с предположението, че стойността му ще се повиши в бъдеще. В случая на ниското общо предлагане на Ethereum, тези инвеститори влияят съществено на цената, тъй като те увеличават търсенето на актива и намаляват неговото предлагане. 

В нашето проучване ние изследваме методи, които проследяват влиянието на тези инвестиции върху крайната стойност на актива. 

\subsubsection{Първоначално предлагане на активи (ICO)} 

Първоначалното предлагане на активи \cite{ico} е форма за набиране на средства за проекти. Екипът създава нов дитигален актив, в който широк кръг инвеститори инвестират. Стойността на актива е пропорционална на успеха на проекта. През 2017 общото кумулативно финансиране на ICO проектите се е увеличило повече от $80$ пъти \cite{ico-funding}. За съжаление, инвестирането в ICO не носи правната защита, която получават традиционните инвестиции, което ги прави рискова инвестиция. 

Вълненията и разочарованията около ICO проектите са основен определящ фактор за дигиталните валути през последната година. Благодарение на средствата за създаване на криптоприложения чрез Ethereum, тази мрежа се е превърнала в най-популярната платформа за набиране на средства чрез ICO. Смята се, че това е основна причина за скока в цената на Ethereum през 2017 г. 

Ние проследяваме дейностите на ICO приложенията в блокчейна, за да преценим тяхното влияние върху стойността на ETH криптовалутата. 

\subsubsection{Влияние на други активи} 
\label{altcoin-interference} 

След Bitcoin са се появили стотици други криптоактиви. Въпреки факта, че те са напълно несвързани и независими една от друга, големи събития в една мрежа и валута могат да доведат до неочаквани промени в други. ICO събитията в Ethereum предизвикаха пикове при много други валути, като Litecoin \cite{litecoin}. 

%we don't track any such data. 
%Should we mention the first sentence? Is it not obvious that it leads to a research ? 
Понастоящем нашите прогнозиращи модели не вземат под внимание намесата на други активи. Нашата цел за по-нататъшно проучване е да включим данни от други блокчейн технологии в първичните ни данни.

\subsubsection{Влияние на медиите} 
\label{media-influence} 

Медийните публикации често оказват силно влияние върху стойността на определени криптоактиви. Пример за това е широко разпространената фалшива новина за инцидент с основателя на Ethereum, Vitalik Buterin \cite{vitalik-death}. Това доведе до временен спад от 4\$ милиарда в стойността на криптовалутата. 

%we don't get such data yet, is that a problem? 
Понастоящем нашите прогнозиращи модели не отчитат влиянието на медиите. Нашата цел в по-нататъшно проучване е да извършим експерименти с дълбоко машинно самообучение въз основа на ``анализ на отношението'' от новини и социални медии, свързани с криптоактиви.

%\subsubsection{Attacks and thefts} 

%Ethereum's smart contract framework is anything but flawless. The immutability and publicity of smart contracts have placed many in concerns that a published contract with flawed code can be attacked and exploited. There have been countless moments of Ethereum's history where similar events have occured. The first major disaster was ``The DAO'' hack, where a hacker stole 50M\$ worth of ETH due to a vulnerability in the contract \cite{dao}. Very recent, and unfortunately much more catastrophic, are two attacks on parity's multi-signature wallet. The first attack was due to a security vulnerability in the contract which resulted in 30M\$ worth of ETH being stolen \cite{parity1}. The second attack happened following the fix of the initial vulnerability, which opened another vulnerability in the process. The result was 300M\$ worth of ETH being completely frozen and unusable, likely forever \cite{parity2}. 

%Other than smart contract related attacks, the usual cryptocurrency thefts still stand. Cases where money are sent to the wrong address, someone reveals the private key of an account or simply fools people into sending him ETH for a promise are a common occurrence. There are no consumer protections and no real way to get money returned, if their current owner doesn't want to. 

%We will track closely smart contract activity, as well as unusual transfers of tokens to increase our prediction accuracy. 



\subsection{Дълбоко машинно самообучение при прогнози за активи} 
Дълбокото машинно самообучение \cite{deep_learning} представлява проектиране на многопластова невронна архитектура и нейното трениране с голямо количество данни. Тази техника е особено полезна при нужда от намиране на корелация или зависимост в голяма набор от данни. Това прави дълбоките мрежи идеални за нашите нужди, понеже ние се опитваме да установим дали можем да намерим корелация между данните в блокчейна и бъдещите характеристики на криптовалутата. 

\section{Източници на данни} 
\label{data-sources} 

За целите на изследването, събираме два вида данни: исторически пазарни данни и първични блокчейн данни. Пазарните данни са агрегирани от няколко борси за търговия на криптовалути, за да се постигне по-широк поглед върху пазарното състояние. Нашите блокчейн данни включват всяка транзакция, изпълнение на криптодоговор и блокчейн събитие през цялата история на Ethereum. Блокчейнът е с размер от стотици гигабайти, като нараства всеки ден. \cite{blockchain-size}. 
%Do I need to point out something like "For details about what we filter out are found on our Github" 
Поради големия размер, ние филтрираме повечето от несъответстващите на нашите изследователски цели първични данни. 

Събрали сме данните за Ethereum блокчейна от неговото начало (08-08-2015), като за всеки блок във веригата ние събираме следните данни: време на създаване, номер (индекс във веригата), миньор (създател на блока), списък с потвърдените транзакции, размер в байтове, трудност при създаване и използваните изчислителни ресурси (газ лимит и използвана газ). 

За всяка транзакция в блок събираме следните данни: адреса на инициатора и получателя, стойността, използваните ресурси (газ) и сумата, платена за единица ресурс (цената на газа). Ние също така симулираме всяко извикване на крипто-договор и събираме всички следи (traces), които то създаде. Следа е всяка контрактна дейност (примерно паричен трансфер, изпълнение на друг контракт или контрактни събития), която не е съхранена на блокчейна. Това също ни помага да наблюдаваме ERC20 ICO активността отблизо.

%do we need to excuse ourselves for not having frequent data? 
Нашите пазарни данни покриват същия период, започвайки от 8-08-2015. Размерът на пазарния тик (честотата на сигналите) е един час. Това са най-честите и най-висококачествени данни, които намерихме като публично достъпни. За всеки тик имаме информация за $open$, $close$, $low$ и $high$ стойностите, както и обемът на търговията до и от валутата. 

Общият размер на нашите филтрирани и компресирани първични блокчейн данни е около 500GB, съдържащ $5,300,000$ блокове с общо $194,000,000$ транзакции и близо \textbf{милиард} следи. Бяха необходими 30 дена за изтегляне на данните и още 14 за обработка, филтриране, форматиране и записване в база данни. 

\section{Извличане на свойства} 
\label{property-generation} 

За да оптимизираме процеса на трениране и да намалим пренасищането (overfit) на нашите невронни модели, ние извличаме най-важните свойства от първични данни. Създадохме набор от свойства, които сме подбрали въз основа на тяхната важност и значение за проблема. За всеки пазарен тик в историческите данни, ние изчисляваме стойността на всяко от избраните свойства. Генерираните свойства са абсолютни стойности. Име на свойство със суфикс ``$\_rel$'' означава, че стойностите му са превърнати в относителни. Пример е данен във Фигура  \ref{propertyGasUsed}. 

Основните свойства, състоящи се от една стойност, които генерираме, са дефинирани в Таблица \ref{properties}. Следващите раздели обясняват по-усъвършенствани концепции за разширяване на нашия набор от свойства. 

\begin{table}[h]
\centering
\begin{tabular}{l|l}
Свойство & Описание \\
\hline
openPrice & Стойността на ETH в началото на тика \\
closePrice & Стойността на ETH в края на тика \\
stickPrice & closePrice-openPrice \\
volumeTo & Обмена на търговията до валутата \\
volumeFrom from & Обмена на търговията от валутата \\
transactionCount & Брой транзакции \\
dappOperations & Брой операции с криптодоговори \\
blockSize & Среден размер на блока в байтове \\
difficulty & Средна трудност за създаване на блок \\
uniqueAccounts & Брой съществуващи акаунти \\
gasLimit & Среден лимит на използваните ресурси \\
gasPrice & Средна цена за една газ единица \\
gasUsed & Средно количество използвани ресурси \\
networkHashrate & Обща мощност на всеки миньор в мрежата \\
ETHSupply & Общ брой ETH единици в циркулация \\
pendingTransactions & Брой транзакции, чакащи изпълнение \\
blockchainGrowth & Ръст на блокчейна в гигабайти \\
\end{tabular}
\caption{\label{properties}Дефиниции на свойствата, пресметнати на базата на първичните ни данни. Свойствата се отнасят за времеви период от един тик.}
\end{table} 

%may be too tiny. 
\begin{figure}[h]
\centering\includegraphics[width=\linewidth]{assets/property_graph}\hfill
\newline
\centering\includegraphics[width=\linewidth]{assets/property_graph_rel}\hfill
\caption{Абсолютните (горе) и относителните (долу) стойности на свойството $gasUsed$ с времето.}
\label{propertyGasUsed}
\end{figure} 

\subsection{Технически индикатори} 

Стойностите на нашите свойства включват значително количество статистически шум, който може да попречи на тренирането. Ние изглаждаме всички наши свойства чрез набор от статистически функции, които се прилагат успешно в редица стратегии за прогнози на пазарни цени. Функциите включват Simple Moving Average ($SMA$) и Exponential Moving Average ($EMA$). Всичките ни функции работят върху 10 тикови интервали. Име на свойство с наставки ``$\_sma$'' и ``$\_ema$'' означава, че стойностите са изгладени от съответната функция. 

\subsection{Дистрибуция на балансите на акаунтите} 
\label{account_balance_distribution} 

Ние взимаме всички активни акаунти в Ethereum в рамките на период от един тик и причисляваме определен номер на група към всеки акаунт въз основа балансовата категория, в която акаунтът попада: 
$$groupN = \lfloor\log_{b} max\rfloor; \hspace{1ex} group = \min(\lfloor\log_{b} bal\rfloor, groupN-1)$$ 

Където $bal$ е балансът на акаунта и $max$ е теоретичният максимален баланс, пресметнат въз основа на константото увеличение на съществувашите ETH активи. Използваме $\log$ скала, защото някои баланси са по-високи от $100\sigma$ от средния баланс. Стойността на $b$ корелира с $groupN$ и съответно с разделителната способност на дистрибуцията. Препоръчваме стойности $\in[1.2; 2]$.

За всяка група изчисляваме общия обем на ETH прехвърлен от, прехвърлен до и общ брой транзакции инициирани от акаунти в групата за определения тик. Ние подреждаме тези стойности в $3 * groupN$ матрица, като резултатът представлява моментна картина на обобщената активност в мрежата за този период от време. Тези стойности са свързани пространствено и имат строг ред. Фигура \ref{account_balance_graph} съдържа визуализиран пример на дистрибуцията. 

\begin{figure}[h]
\centering\includegraphics[width=\linewidth]{assets/distributions/accountBalanceDistribution_log1_2}
\centering\includegraphics[width=\linewidth]{assets/distributions/accountBalanceDistribution_log2}
\caption{Примери с $b$ $1.2$ (горе) и $2$ (долу). Оста $X$ представлява номера на групата. Стойностите на $Y=0$ са прехвърлен обмен до, $Y=1$ са прехвърлен обмен от и $Y=2$ са брой транзакции. Всички стойности да допълнително скалирани с $\log_2$.}
\label{account_balance_graph}
\end{figure} 

\subsection{Дистрибуция на броя акаунти} 
\label{account_number_distribution} 

За да увеличим пространствената информация в нашите данни, нашите свойства трябва да бъдат матрици с по-висока размерност. Също така искаме и да обработваме данни за повече от един конкретен пазарен тик, за да направим цялостна моментна картина на състоянието на мрежата. За всеки пазарен тик вземаме всички съществуващи Ethereum акаунти и ги групираме на базата на две черти: 
$$groupN_{1,2} = \lfloor scl_{1,2}(max_{1,2})\rfloor$$
$$group_{1,2} = \min(\lfloor scl_{1,2}(feat_{1,2})\rfloor, groupN_{1,2}-1)$$

%explain the features which we track. Give us an example configuration 
Чертите, чрез които групираме акаунтите, са $feat_{1,2}$ . Примери за черта включват секунди от последната активност, баланс, общ обем на ETH през последните 30 дни и средна стойност на транзакцията. Стойността на теоретичната максимална стойност на конкретната черта е $max$. Най-добрата скалираща функция ($scl$) за нашите цели е логаритъм ($y = \log_{base} x$). Понеже ние начисляваме два номера на групи за всеки акаунт, ние имаме два набора от независими групи (обозначени с индекси $1$ и $2$ ). Всеки набор от групи има различни стойности за $feat$, $scl$ и $groupN$. Ние създаваме матрица, където стойността в $[i,j]$ е $\log_2$ от броя акаунти, които са начислени към групите $i$ и $j$. Фигура \ref{account_number_example} съдържа примерни конфигурации. 

\begin{figure}[h]
\centering\includegraphics[width=\linewidth]{assets/distributions/balanceLastSeenDistribution_log1_2}
\centering\includegraphics[width=\linewidth]{assets/distributions/contractVolumeInERC20Distribution_log2_v2_stateless}
\caption{\textbf{balanceLastSeenDistribution (ляво)}: дистрибуция на всички съществуващи акаунти на базата на техния баланс ($Y$) и секунди от последната активност ($X$), и двете с $\log_{1.2}$ скала. Видео анимация от стойностите на дистрибуцията може да бъде намерена \href{https://youtu.be/czfBa75HuWs}{тук: youtu.be/czfBa75HuWs}. \textbf{contractVolumeInERC20Distribution (дясно)}: дистрибуция на скорошно активни ICO криптодоговори на базата на входния им обмен ($Y$) и брой операции с тях ($X$), с $\log_2$ скала.}
\label{account_number_example}
\end{figure} 

Друга конфигурация е \textbf{contractBalanceLastSeenDistribution} - разпределение на криптодоговори на базата на същите черти и скала, както balanceLastSeenDistribution. 

Други дефиниции и примери са на разположение на \href{https://goo.gl/zDDxxA}{Wiki страницата на проекта: goo.gl/zDDxxA}.

\section{Създаване на датасет} 
\label{dataset-generation} 

\subsection{Цел на прогнозата} 
%not sure if 51% attacks should be mentioned 
Нашата цел на прогнозата е стойността на едно или няколко свойства в тика, който следва текущия момент. Освен движения на цената, нашите стратегии могат да бъдат приложени при прогнози за брой нови потребители, обмен на търговията, брой транзакции и дори забавяния на мрежата (сериозен проблем в контекста на скорошни събития \cite{blockchain-clogging}). 
%or possibly attempts of 51\% attacks \cite{51attack}. 

Нашите експерименти са съсредоточени главно върху прогнозирането на движенията на цените и брой нови портебители. 

\subsection{Нормализация} 
\label{normalization} 
%a single value cannot have zero mean and equal variance 
Поради особенностите при дигитални изчисления с реални числа, всяка стойност в нашия датасет трябва да бъде нормализирана. Някои алгоритми скалират до малък интервал, като $\in [0; 1]$, а други не са ограничени в интервал и създават последователности с нулева средна стойност и равна дисперсия. Предлагаме следните стратегии за нормализиране в зависимост от ситуацията: 

$$basic_i = \frac{x_i - min(x)}{(max(x) - min(x))}$$ 

Използваме тази основна min-max скала, за да вместим независими последователности с еднозначни стойности до интервала $\in [0; 1]$. 

$$around\_zero_i = \frac{x_i + max(\lvert max(x) \rvert, \lvert min(x) \rvert)}{2*max(\lvert max(x) \rvert, \lvert min(x) \rvert)}$$ 

Скалираща функция, като $basic$, която вмества положителни и отрицателни стойности в $(0.5; 1]$ и $\in [0; 0.5)$ съответно. Използваме тази скала, когато нормализираме последователности със стойности от различен знак. 

%do I need to specify what is std? 
$$image_i = (x_i - \frac{1}{n}\sum_{t=1}^{n}x_t) * \frac{1}{std(x)}$$ 

Нормализация без интервал, която създава последователност с нулева средна стойност и еднаква дисперсия. Ние я използваме, когато нормализираме пространствените последователности, като дефинираните в Секция \ref{account_number_distribution}. 
%$$local_i = \frac{win_i}{win_0} - 1$$ 

%Local normalization based on the first element of a window of values. As it does not depend on the whole sequence, it can normalize future values without issue. 
%we don't use sigmoid. Remove it? 
%$$sigmoid_i = \frac{1}{1 + \exp(-arr_i)}$$ 

%Non-linear normalization function that provides consistent normalization no matter the sequence. We recommend this to be used with relatively small values, as normalizing large enough values results in a practically indistinguishable difference in the output value. 
Всяко свойство в нашия набор от данни е различна последователност и съответно е нормализирано отделно с избран алгоритъм. Метод за автоматично определяне на алгоритъма за всяко свойство се нарича $prop$. Използва се $basic$ скала, ако стойностите на определеното свойство са абсолютни. В противен случай се използва $around\_zero$ скала. 

Последователности със стойности над $10 \sigma$ са първо скалирани с логаритъм преди нормализация. Повечето от гореспоменатите стратегии нормализират въз основа на $\min$ и $\max$ стойности на последователността и бъдещи стойности на поредицата могат да надхвърлят тези граници. Частично решение на проблема е, ако се използват само относителни стойности. При нашите експерименти, относителните стойности резултират в по-нисък overfit и по-висока генерализация на нашите дълбоки мрежи. Ние също така използваме техника, наречена normalization space overprovisioning, която увеличава стойностите на $\min$ и $\max$ с даден процент, за да се намали вероятността бъдещи стойности да надхвълрят границите. 
%The problem of future values can be solved completely by using $local$ normalization, but that is the best algorithm in all cases. 
Всички гореспоменати методи за справяне с проблема могат да бъдат използвани едновременно. 

\subsection{Модели на датасет} 
\label{dataset-models} 
Датасет е последователност от елементи, състоящи се от входове (стойности на свойства) и очаквани изходи (прогнози). Ние предлагаме няколко начина за моделиране (подреждане на нормализираните стойности на свойствата) на датасет елементите. Всички наши модели имат следните общи черти - за да се създаде един датасет елемент, ние  минаваме с плъзгащ прозорец (с конфигурируем размер $n$) през стойностите на избрани свойства: 

$$x \in [0, n-1]; \hspace{1ex} y \in [0, propN-1]$$ 
$$win_{x,y} = propY_{x+step}$$ 
$$tar = propT_{n+step}$$ 

Където $prop0,1,2,..,y$ е списъкът от избрани свойства с дължина $propN$. За всеки датасет елемент, $step$ се увеличава с $1$. Целта на прогнозата е свойството $propT$. Очакваният изход при този елемент от датасет е $tar$. 

Начинът, по който един прозорец от стойности е структуриран в елемент от датасет, зависи от избрания модел на датасет. Ние предлагаме следните начини за моделиране: 

\subsubsection{Матричен модел} 

Репрезентацията на матричния модел наподобява двуизмерния вход на LSTM мрежата. Един датасет елемент е създаден по следния начин: 

$$sam_{x,y} = norm_y(win_{x,y})$$ 

Където $norm_y$ е избраната стратегия за нормализиране на конкретното свойство. 

Таблица \ref{matrix_model_table} визуализира структурата на един датасет елемент. 

%this may be useless 
%The format has a lot in common with LSTM network's input shape, which is ($time\_steps$, $features$). For our case, each $feature$ is a property and each property value is a $time\_step$. 

\begin{table}[h]
\centering
\begin{tabular}{l|r|r|r}
Property & Value $0$ & Value $1$ & ... Value $n-1$ \\\hline
Close value & 349\$ & 358\$ \\
Number of TXs & 2876 & 1583 \\
Operations with Dapps & 459 & 508 \\
\end{tabular}
\caption{\label{matrix_model_table}Примерна структура на елемент, създаден с матричния модел.}
\end{table} 

\subsubsection{Слоеви модел} 
\label{stacked-model} 

\begin{wrapfigure}{R}{0.5\linewidth}
\centering\includegraphics[width=\linewidth]{assets/stacked_model}
\caption{Визуализация на слоевия модел.}
\label{stacked_model_example}
\vspace{0pt} %workaround, because wrapfigure hates the float package
\end{wrapfigure} 

Слоевият модел (Фигура \ref{stacked_model_example}) наподобява 3D входа на конволюционната невронна мрежа и нейното пространствено възприятие. 
Всички стойности на свойствата от същия времеви момент са подредени в 2D пространство, образувайки един слой. Дължината на прозореца $n$ обозначава броя на слоевете, които подредени един върху друг образуват изображение с $n$ цветови канала. Форматът на елемент от датасета е ($height$, $width$, $n$). Размерностите $width$ и $height$, както и подредбата на стойностите в слоевете са конфигурируеми. Този модел може най-ефективно да представя пространствени свойства, като дефинираните дистрибуции в секции \ref{account_balance_distribution} и \ref{account_number_distribution}. 

\vspace{1pt} %to move the title of the next section to the next page 

\section{Създадени датасети} 
\label{generated-datasets} 

Дефинираме няколко варианта на датасет, на базата на които провеждаме нашите експерименти. Най-подходящият интервал от време за нашите датасети е от 2017-03-01 до 2017-11-01. Този диапазон обхваща най-големите флуктуации в историята Ethereum, широкоразпространената фалшива новина за Ethereum \cite{vitalik-death} и пика на ICO проектите \cite{ico}. 

%we don't include any stateful LSTM experiments. No need to specify warmup dataset 
Всеки датасет е разделен на $train$ и $test$ датасети.
%Първият месец от интервала е запазен за $warmup$ датасета. Той се използва само при нашите stateful LSTM експерименти и предназначението му е да докара паметта на мрежата до стартово състояние преди тренирането.
Първите 7 месеца от интервала изграждат $train$ набора от данни, въз основа на който се извършва трениране на невронната мрежа. Последният месец е утилизиран от $test$ датасета, използван за оценка на вече тренирана мрежа. 

Датасети $1$ до $4$ не включват блокчейн данни и се използват като база за сравнение. Размерът на прозореца ($win$), целта на предсказване и нормализацията ($Norm$) са посочени в експериментите. 

%multiple prediction targets? 
\begin{table}[h]
\centering
\begin{tabular}{l|p{6.0cm}|r}
setN & Свойства в датасет & Модел \\\hline
1 & volumeFrom, volumeTo & matrix\\\hline
2 & volumeFrom\_rel, volumeTo\_rel & matrix\\\hline
3 & highPrice, volumeFrom, volumeTo & matrix\\\hline
4 & highPrice\_rel, volumeFrom\_rel, volumeTo\_rel & matrix\\\hline
5 & accountBalanceDistribution & matrix\\\hline
6 & balanceLastSeenDistribution & stacked\\\hline
7 & contractBalanceLastSeenDistribution & stacked\\\hline
8 & balanceLastSeenDistribution, contractBalanceLastSeenDistribution, contractVolumeInERC20Distribution, accountBalanceDistribution & stacked\\
\end{tabular}
\caption{\label{dataset_table}Дефинициите на нашите датасети. Свойства с наставка ``\_rel'' са относителни стойности.}
\end{table} 

\section{Генетичната рамка}
\label{genetic-framework}

Дълбоките модели обикновено имат стотици хипер- и мета-параметри относно невронната архитектура, параметри за трениране и конфигурация на датасет, всеки от които трябва да бъде настроен индивидуално. Броят възможните конфигурации е твърде голям в сравнетие с това което ние можем да оптимизираме ръчно. Нашата рамка за прогнози позволява автоматична настройка на някои хипер-параметри със сесии от трениране, оценяване и съответна промяна в параметрите. Тази техника е приложена в нашите експерименти. За да автоматизираме процеса, ние избрахме да създадем генетична рамка, която има за цел да автоматизира генерирането на невронна архитектура и конфигурирането на хиперпараметрите и на датасета чрез създаване на множество агенти за постигане на дадена прогнозна задача.

Агентът представлява дълбока мрежа и съответните параметри за тренирането му. Агент се създава от геном, състоящ се от набор от хромозоми. Всяка хромозома представлява масив от цели числа с дължина, зависеща от хромозомния тип. Примерни типове включват конфигурация на входните данни, параметри за трениране и конкретен слой на дълбока невронна архитектура със своите параметри (например $Conv2d$, $LSTM$). Създадохме $JSON$ спецификация за нотирането на всяка невронна архитектура и $converter$, който създава $JSON$ от геном. Изходният $JSON$ се предава на $parser$, който създава и връща дълбокия модел, готов за трениране.

\begin{figure}
\centering\includegraphics[width=\graphwidth]{assets/genetic_engine}\hfill
\caption{Структурата на нашата генетична рамка}
\label{genetic-framework-scheme}
\end{figure}

Фигура \ref{genetic-framework-scheme} визуализира действията в рамката. Първоначално се създава популация от $n$ индивиди (геноми) със случайни хромозоми. Повечето стойности на хромозомите имат ограничения (например, размерът на слой не може да бъде отрицателна стойност). Всеки индивид преминава през първоначална проверка, която променя хромозомите, за да влязат в рамките на всички граници. След това индивидите са преобразувани в нашия $JSON$ формат и са превърнати в дълбоки модели. Ако създаването на модел се провали (например невалидна комбинация от слоеве), даденият индивид не продължава нататък в процеса. Създадените агенти се тренират посредством Reinforcement Learning за да научат стратегия на търгуване като подават сигнали за "купуване" и "продаване" на съответният актив.
Свойствата, включени в датасета на индивида, са обозначени в неговия геном. След тренирането, всеки агент е оценен и класиран със своя резултат, който е базиран на резултатите от симулирано търгуване върху тестови набор от данни. 

Набор от нови индивиди се създава чрез произволни бинарни мутации в стойностите на хромозомите, случайно добавяне/премахване на хромозоми, Two-point crossover \cite{twopoint-crossover} и Uniform crossover \cite{uniform-crossover} от двама родители, избрани чрез Fitness proportionate selection и Tournament selection. Индивидите с най-добра производителност $x\%$ не претърпяват мутации, а най-лошите се премахват, за да се запази стабилен брой на популацията. Полученият набор от геноми се преобразува в $JSON$ и се създава агент за всеки, който след това се тренира. Този алгоритъм се повтаря до намирането на индивиди с оптимална производителност.

Нашата генетична рамка в момента е в процес на разработка и засега не участва в оформянето резултатите в проучването ни.
\if\showlinks1
Тя е с отворен код и е качена на \href{https://github.com/obecto/gattakka}{следния адрес: https://github.com/obecto/gattakka}
\fi

\section{Измервания на грешка} 
\label{measures} 

Използваме следните мерки за оценка на ефективността на мрежата: 

$$MSE = \displaystyle\frac{1}{n}\sum_{t=1}^{n}err_t^2;
\hspace{2ex} RMSE = \sqrt{\displaystyle\frac{1}{n}\sum_{t=1}^{n}err_t^2};
\hspace{2ex}R^2 = 1-\displaystyle\frac{\sum_{t=1}^{n}err_t^2}{\sum_{t=1}^{n}null_t^2}
$$ 

$$%custom = \displaystyle\frac{1}{n}\sum_{t=1}^{n}\frac{\lvert err_t \rvert}{min(pred_t, true_t)};
\hspace{2ex}sign = \frac{t}{t+f}
\hspace{2ex}err_t = pred_t - true_t;
\hspace{2ex}null_t = 0.5 - true_t$$ 

Където $n$ обозначава броя на елементите в нашия набор от данни, $pred$ и $true$ са съответно списъци на прогнозираните и очакваните стойности. Броят на правилно и неправилно погнозираните знаци на промяната на целта е съответно $t$ и $f$. 

Мерките $R^2$ и $sign$ представляват точност и нашата цел е повишим стойността им, която е $\leq 1$. При $R^2$ точността на нашия модел се сравнява с тази на $null$ модела - такъв, който връща една и съща прогноза ($0.5$ в случая) независимо от входа. $MSE$ и $RMSE$ са мерки за грешка, които трябва да смъкнем като стойност. 
%In efforts to observe our network's performance from different angles, we have created our own error function, called $custom$. 
Използваме $MSE$ като $loss$ функцията при трениране. Останалите мерки са използвани за оценка на вече тренирана мрежа. 
%null model for predicting absolute value? 

\section{Невронни архитектури} 
\label{networks} 
За нашите прогнози сме създали Long Short-Term Memory (LSTM) \cite{LSTM} и конволюционен (CNN) модели. Техните невронни архитектури са показани във Фигура \ref{models}.
LSTM мрежите са известни със своя успех при обработка на времеви последователности от данни и би било интересно да се види как те работят нашите датасети.
%LSTM мрежата може да бъде stateful и stateless. Stateless моделите нулират паметта си след всеки входен елемент на дадасета, докато stateless мрежите си запазват състоянието. 
База за сравнение на нашите експерименти с блокчейн данни е LSTM модел, трениран върху пазарни данни. Тъй като експериментираме с дистрибуции (Секции \ref{account_balance_distribution} и \ref{account_number_distribution}), които имат стриктна подредба в пространството, ние проучваме и конволюционните мрежи, които са известни с техния успех при изображения и пространствени данни. 

\begin{figure}[h]
\centering
\includegraphics[width=\linewidth]{assets/architectures_short_nodnn}
\caption{Архитектурите на нашите LSTM и Конволюционни модели съответно.}
\label{models}
\end{figure} 

\section{Експерименти} 

Експериментите са проведени на базата на нашите дефинирани датасети (Секция \ref{generated-datasets}). Допълнителни експерименти могат да бъдат открити на \href{https://goo.gl/WxnsG1}{Wiki страницата на проекта: goo.gl/WxnsG1}. Експериментите са групирани според цел на прогнозата. Оценяването на мрежите се извършва след обръщането на нормализацията на прогнозираните стойности. Долупосочените експерименти са най-добрите от нашите хиляди първоначални експерименти. Всички измервания освен $sign$ са непосредствено несравними между експерименти с различни цели, защото разчитат на разстоянието между графиките на прогнозите и на действителните стойности. 

Открили сме, че оптималните параметри за трениране са $batch\_size$ от $16$, $1e^{-5}$ $learning\_rate$ и използване на Adam оптимизатора \cite{adam}. Всички наши мрежи са тренирани с тези параметри. 

Тренираните мрежи от експериментите, заедно с детайна история на измерванията ни за грешка по време на тренирането и визуализации на изпълнението, са на разположение на \href{https://goo.gl/RzqEB9}{Wiki страницата на проекта: https://goo.gl/RzqEB9}.

\subsection{Прогнози за цена ($highPrice$)} 
\label{highPrice_exp} 

\begin{table}[h]
\centering
\begin{tabular}{l|r|r|r|r|r|r|r}
$N$ & $setN$ & $win$ & $Norm$ & $Netw$ & $RMSE$ & $R^2$ & $sign$ \\\hline
%matrix-volumeFrom_rel,volumeTo_rel-highPrice-pixel-24w.pickle.pickle
1 & 2 & 24 & image & LSTM & 90.4185 & 0.9131 & 0.5258\\
%matrix-highPrice,volumeFrom,volumeTo-highPrice-property-8w.pickle.pickle
2 & 3 & 8 & prop & LSTM & 5.1060 & 0.9997 & 0.5095\\
%matrix-accountBalanceDistribution-highPrice-pixel-24w.pickle.pickle
3 & 5 & 24 & image & LSTM & 21.9306 & 0.9948 & 0.5054\\
%stacked-balanceLastSeenDistribution_cpp_log2-highPrice-pixel-104w.pickle.pickle
4 & 6 & 104 & image & CNN & 16.2167 & 0.9972 & 0.5115\\
%stacked-balanceLastSeenDistribution_cpp_log2-highPrice-pixel-8w.pickle.pickle
5 & 6 & 8 & image & CNN & 21.2845 & 0.9951 & 0.5033\\
%stacked-contractBalanceLastSeenDistribution_log2_v2-highPrice-property-104w.pickle.pickle
6 & 7 & 104 & prop & CNN & 83.1030 & 0.9265 & 0.5290\\
%stacked-contractBalanceLastSeenDistribution_log2_v2-highPrice-property-24w.pickle.pickle
7 & 7 & 24 & prop & CNN & 82.2199 & 0.9280 & 0.5367\\
\end{tabular}
\caption{\label{highPrice_table}Резултатите от експериментите за прогнози за цена. Измерванията са най-добрите стойности от всички тренирани епохи.}
\end{table} 

Експеримент $2$ прогнозира въз основа на пълни пазарни данни (цената и обмена на търговията), докато експеримент $1$ прогнозира само на базата на обмена на търговията. Грешката на експ. $2$ е драстично по-ниска, понеже мрежата всъщност не прогнозира, а връща предишната цена, подадена на входа (горната част на Фигура \ref{1_2_highPrice}). Това е лесен начин мрежата да намали грешката си. В експ. $1$ мрежата няма достъп до предишната цена и е принудена да намери коректно решение. Всички експерименти със CNN не включват предишни цени като входни данни.

\begin{figure}[h]
\centering
\includegraphics[width=\graphwidth]{assets/1_highPrice}
\includegraphics[width=\graphwidth]{assets/2_highPrice}
\caption{$highPrice$: Тестовите резултати на експ. $1$ (горе) и експ. $2$ (долу).}
\label{1_2_highPrice}
\end{figure} 

Експ. $3$ постига ниска грешка, въпреки че не използва пазарни данни. Мрежата е по-способна да прогнозира правилните движения на стойността (Фигура \ref{3_highPrice}). Добавените блокчейн данни данни намаляват грешката с 330\% в сравнение с експ. $1$.

\begin{figure}[h]
\centering
\includegraphics[width=\graphwidth]{assets/3_highPrice_big}
\caption{$highPrice$: Резултатите на експ. $3$.}
\label{3_highPrice}
\end{figure} 

Експ. $4$ използва повече блокчейн пространствени данни и в комбинация със CNN води до най-ниските ни грешки за тази цел (допълнително подобрение от 35\% спрямо експ. $3$). Въпреки високата грешка, експ. $7$ достига високата знакова точност. Тези експерименти показват, че блокчейн данните подобряват прогнозите и също така, че CNN е най-добрата мрежа за намиране на модели в тях. Конволюционните активации от експ. $4$ могат да бъдат намерети визуализирани на \href{https://goo.gl/etAaod}{Wiki страницата на проекта: goo.gl/etAaod}.

Високите грешки при експ. $6$ и $7$ демонстрират колко неефективно е пространствените дистрибуции да бъдат нормализирани с $prop$ скала. Силно препоръчваме $image$ нормализация при такива данни. 

\subsection{Прогнози за относителна цена ($highPrice\_rel$)} 

\begin{table}[h]
\centering
\begin{tabular}{l|r|r|r|r|r|r|r}
$N$ & $setN$ & $win$ & $Norm$ & $Netw$ & $RMSE$ & $R^2$ & $sign$ \\\hline
%matrix-volumeFrom,volumeTo-highPrice_rel-property-104w.pickle.pickle
1 & 1 & 104 & prop & CNN & 2.3652 & -0.0031 & 0.5502\\
%matrix-highPrice_rel,volumeFrom_rel,volumeTo_rel-highPrice_rel-pixel-104w.pickle.pickle
2 & 4 & 104 & image & CNN & 2.3019 & 0.0498 & 0.4932\\
%stacked-contractBalanceLastSeenDistribution_log2_v2-highPrice_rel-pixel-24w.pickle.pickle
3 & 7 & 24 & image & CNN & 2.2825 & 0.0513 & 0.5340\\
%stacked-balanceLastSeenDistribution_cpp_log2,contractBalanceLastSeenDistribution_log2_v2,contractVolumeInERC20Distribution_log2_v2_stateless,accountBalanceDistribution-highPrice_rel-pixel-8w.pickle.pickle
4 & 8 & 8 & image & CNN & 2.2878 & 0.0461 & 0.5512\\
%stacked-balanceLastSeenDistribution_cpp_log2,contractBalanceLastSeenDistribution_log2_v2,contractVolumeInERC20Distribution_log2_v2_stateless,accountBalanceDistribution-highPrice_rel-property-104w.pickle.pickle
5 & 8 & 104 & prop & CNN & 9.1956 & -14.2060 & 0.5466\\
\end{tabular}
\caption{\label{highPrice_rel_table}Резултати.}
\end{table} 

Прогнозите за относителна цена принуждават мрежата да намери коректно решение, понеже не може да измами като върне предишна цена като прогноза (както се вижда при експ. 2 в Секция \ref{highPrice_exp}). Поради това разликата в грешката при експ $1$ и $2$ не е голяма. 

Експеримент $4$ води до най-ниската грешка и нашата най-висока знакова точност. Точността $sign$ е близо до тази на експ. $1$, но CNN предоставя по-висока $R^2$ точност. От графиката на прогнозите (Фигура \ref{4_highPrice_rel}) се вижда, че въпреки резултатите, мрежата не е много уверена в стойността на промяната на цената. Това предполага, че за да се намали грешката е необходимо да се оптимизират хиперпараметрите и мрежовата архитектура. Датасетът за експ. $4$ съдържа повече пространствена информация, като включва 4 пространствени дистрибуции и това се вижда в повишената $sign$ точност. 

\begin{figure}[h]
\centering
\includegraphics[width=\graphwidth]{assets/4_highPrice_rel_big}
\caption{$highPrice\_rel$: Тестовите резултати от експ. $4$.}
\label{4_highPrice_rel}
\end{figure} 

\subsection{Прогнози за брой нови потребители ($uniqueAccounts\_rel$)} 

\begin{table}[h]
\centering
\begin{tabular}{l|r|r|r|r|r|r}
$N$ & $setN$ & $win$ & $Norm$ & $Network$ & $RMSE$ & $R^2$ \\\hline
%matrix-volumeFrom_rel,volumeTo_rel-uniqueAccounts_rel-property-104w.pickle.pickle
1 & 2 & 104 & prop & LSTM & 1139.972426 & 0.737456\\
%matrix-volumexFrom,volumeTo-uniqueAccounts_rel-property-104w.pickle.pickle
2 & 1 & 104 & prop & LSTM & 718.971374 & 0.895567\\
%stacked-contractBalanceLastSeenDistribution_log2_v2-uniqueAccounts_rel-pixel-8w.pickle.pickle
3 & 7 & 8 & image & CNN & 812.303885 & 0.864637\\
%stacked-balanceLastSeenDistribution_cpp_log2-uniqueAccounts_rel-pixel-24w.pickle.pickle
4 & 6 & 24 & image & CNN & 639.336022 & 0.916289\\
%stacked-balanceLastSeenDistribution_cpp_log2,contractBalanceLastSeenDistribution_log2_v2,contractVolumeInERC20Distribution_log2_v2_stateless,accountBalanceDistribution-uniqueAccounts_rel-pixel-8w.pickle.pickle
5 & 8 & 8 & image & CNN & 622.716696 & 0.920449\\

\end{tabular}
\caption{\label{uniqueAccounts_rel_table}Резултати.}
\end{table} 

Тези експерименти имат за цел да покажат как блокчейн данните могат да бъдат използвани за изграждане на прогнози на други черти на криптовалутата, като примерно как ще се промени общественият интерес към нея. 

Знаковата точност е без значение в този случай, понеже броят на потребителите винаги се увеличава. 

Експериментите с пазарни данни ($1$ и $2$) водят до най-високата грешка и най-ниската точност. При прогнозиране на факти за самия блокчейн, много повече стойност може да се извлече от блокчейн данните, както се вижда със CNN резултатите. Експеримент $5$ (Фигура \ref{5_uniqueAccounts_rel}) дава впечатляващи резултати при всички измервания, което вероятно се дължи на богатата пространствена информация съдържаща 4-те пространствени дистрибуции в датасета. 

\begin{figure}[H]
\centering
\includegraphics[width=\graphwidth]{assets/5_uniqueAccounts_rel_big}
\vspace{-0em}
\caption{$uniqueAccounts\_rel$: Тестовите резултати на експ. $5$.}
\label{5_uniqueAccounts_rel}
\end{figure}  

\section{Резултати} 

Допълнителни резултати могат да бъдат намерени на \href{https://goo.gl/WxnsG1}{Wiki страницата на проекта: https://goo.gl/WxnsG1}.

С нашите експерименти, ние наблюдавахме проблема от няколко гледни точки, тренирайки множество мрежи на множество датасети и оценявайки прогнозите с различни измервания за грешка и точност. 

Резултатите ни показаха, че Ethereum е твърде променлива и непостоянна криптовалута, за да бъде предвидена добре въз основа само на пазарни данни. 

Когато използвахме блокчейн данни, ние постигнахме 330\% по-ниска грешка в сравнение с грешката при използване на данни за обема на търговията. С нашата конволюционна архитектура, пространствени дистрибуции на акаунти, image нормализация и пространствено моделиране на датасета, ние намалихме грешката с допълнителни 35\% и времето за трениране десеторно. 

Нашите най-добри цялостни резултати са постигнати с блокчейн данни, което потвърждава първоначалната ни хипотеза, че този вид данни могат да подпомогнат прогнозите. Основните ни свойства от блокчейна (дефинирани в Таблица \ref{properties}) не са достатъчни за висока точност на прогнозите. Тези констатации обясняват ниските точности в проучването на екипа от университета Станфорд за Bitcoin прогнози \cite{stanford-predictions}. Най-стойностният вид блокчейн информация се явяват пространствените дистрибуции на акаунти (Секция \ref{account_number_distribution}). Те извличат най-много смисъл от първичните ни блокчейн данни. Най-добрият ни датасет съчетава всички 4 от нашите пространствени дистрибуции (Номер $8$ в Таблица \ref{dataset_table}), като се използва слоевият модел (Секция \ref{stacked-model}). Най-добрата цел за прогноза е относителна $highPrice$, защото тя принуждава моделите да намерят същинско решение на проблема. Най-добрата невронна мрежа за намиране на правилни връзки и корелации в датасета ни е нашият конволюционен модел, трениран с Adam оптимизатора \cite{adam}. Препоръчваме $batch\_size$ от 16, което осигурява баланс между времето за трениране и генерализацията на мрежата. Има начини да се увеличи точността при висок $batch\_size$ \cite{accurate-large-batch}, но по-ниска стойност винаги води до по-висока точност. 

Нашето блокчейн решение включва много повече параметри, отколкото са при стандартно решение с пазарни данни и следователно броят възможни конфигурации е експоненциално по-голям. Трябва да се проведат повече експерименти с различни архитектури и хиперпараметри, преди да бъдем заключителни в резултатите си.

\section{Техническа реализация} 

За нашия експеримент ние създадохме и документирахме гъвкава рамка, която позволява изграждане на стратегии за прогнозиране на всяка черта на всеки блокчейн на базата на всякакви данни. Нашите свойства, модели за датасети, стратегии за нормализация и гореспоменатите техники са реализирани и предоставени с отворен код в нашата имплементация на тази рамка за криптовалутата Ethereum.

Рамката е разделена на множество инструменти, които управляват изтеглянето и съхранението на данни, пресмятането на свойства, създаването на датасети, тренирането и оценяването на невронни мрежи:

\begin{itemize} 
\item \textbf{Модул за извличане на данни}: отговаря за връзката с източниците на данни (като описаните в Секция \ref{data-sources}) - изтегля, валидира и съхранява първичните данни;

\item \textbf{Модул за съхранение на данни}: Приема и извършва обработка на първичните данни, като филтрира ненужните данни за нашето изследване и запазва останалата част като времева последователност в база данни. За бърз достъп до данните по даден интервал от време, те са разделени на времеви сегменти;

\item \textbf{Модул за пресмятане на свойства}: Чете запазените първично обработени данни, пресмята и съхранява стойностите на свойствата (дефинирани в Секция \ref{property-generation});

\item \textbf{Модул за създаване на датасет}: Създава датасет, като нормализира избрани пресметнати свойства и ги подрежда в простнарството спрямо избран модел за датасет (процесът е описан в Секция \ref{dataset-generation});

\item \textbf{Модул за трениране и оценяване}: Тренира избрана невронно мрежова архитектура на базата на създаден датасет и измерва точността на тренираната мрежа. Нашите предложени архитектури са в Секция \ref{networks}, а измерванията за грешка и точност са описани в Секция \ref{measures}. 
\end{itemize} 

\subsection{Автоматизирани тестове} 

Създали сме unit и интеграционни тестове за всички наши инструменти, където е приложимо. Целта на това е да гарантираме, че набор от данни създаден чрез тези инструменти винаги е с очакваните и правилни стойности. 

\section{Технологии} 

\begin{enumerate} 
\item \textbf{JavaScript} се използва при модула за извличане на данни; 
\item \textbf{Web3 API} позволява извличането на блокчейн информация от локален Ethereum node; 
\item \textbf{Node.js} изгражда връзката с други източници за останалата част от първичните ни данни; 
\item \textbf{Python} е главният език при всички останали модули; 
\item \textbf{Pandas} предоставя гъвкави структури на данни и високоскоростни инструменти за анализ на данни в Python; 
\item \textbf{MongoDB} е базата данни, в която съхраняваме данните си във всички етапи от обработката; 
\item \textbf{Arctic} е предоставя ефективно структуриране на времеви серии и инструменти за работа с тях. Използва се в хедж фондове; 
\item \textbf{Tensorflow} е библиотеката за дълбоко машинно самообучение, която най-често се използва при проучвания и разработка на дълбоки мрежи;
\item \textbf{Keras} е рамка за създаване на дълбоки невронни мрежи в език от високо ниво, като това позволява бързо прототипизиране на архитектури;
\item \textbf{Scala} е използвана в основата на генетичната рамка;
\item \textbf{Akka} е рамка за Актьор модела, имплементиран в нашата генетична рамка, която позволява скалиране на оптимизациите на агенти на множество отделни компютри едновременно.
\end{enumerate} 


\section{Github repository} 
%пренасяне на нов реД? 
Нашата рамка и нейната имплементация за Ethereum са с отворен код под MIT лиценз. \href{https://github.com/Zvezdin/blockchain-predictor}{GitHub страницата на проекта може да бъде намерена тук: https://github.com/Zvezdin/blockchain-predictor}.

Страницата включва техническа документация за проекта, включително инструкции за настройка, употреба и стъпки за възпроизвеждане на нашите резултати. 

Създадена е и Wiki страница за проекта, която включва допълнителна информация за проучването \href{https://github.com/Zvezdin/blockchain-predictor/wiki}{и може да бъде намерена тук: https://github.com/Zvezdin/blockchain-predictor/wiki}.

\section{Бъдещо развитие} 

По време на нашето проучване ние не само оценихме няколко модела дълбоки невронни мрежи, но и изградихме гъвкава рамка за събиране, обработка и съхранение на блокчейн и пазарна информация. С помощта тази рамка, по-голямата част от нашата по-нататъчна работа по проучването се състоеше от изпробване на различни мрежови архитектури и мета-параметри. Макар, че този процес сам по себе си е предизвикателство и изисква дълбоко познание и творческо мислене, ние сме развълнувани от възможностите да експериментираме с автоматизацията му. 

Две скорошни публикации на Google Research \cite{automl-genetic} \cite{automl-rl} показват, че с достатъчно изчислителна мощност можем да създадем ``контролер'' алгоритъм, който да генерира невронни модели за класифицирането на CIFAR10 датасета \cite{cifar-10}. Тези модели достигат производителност, съизмерима с най-модерните модели, проектирани от хора. Авторите подчертават огромната изчислителна мощност, необходима за постигането на тези резултати, която е била от порядъка на 10\textsuperscript{20} операции. За сравнение, повечето приближения на мощта на човешкия мозък го поставят между petascale (10\textsuperscript{15}) и exascale (10\textsuperscript{18}) операции в секунда \cite{brain-processing-power}.

Вече сме изградили основата на нашата генетична рамка и следващите стъпки са към прилагането й в нашите експерименти. Нашата амбиция е да развием генетичната рамка в децентрализирана архитектура, която позволява на отдалечени системи да предоставят изчислителна мощ на ``контролер'' алгоритми за трениране и оценяване на индивидуални модели на дълбоки мрежи. В такава система могат да бъдат интегрирани децентрализираните приложения на Ethereum за осъществяване на децентрализиран пазар за трениране и оптимизация на модели на невронни мрежи. 

Следим отблизо развитието на Ethereum по въпроса с приемането към алгоритъма ``Proof of Stake'', който би могъл да обезсмисли използването на графични карти за осигуряване на ``Proof of Work''. Понастоящем такива ``mining`` компютри консумират огромно количество електроенергия \cite{electricity-for-mining}, която се хаби само за сформирането на консенсуса в мрежата. След внедряването на ``Proof of Stake'' алгоритъма, огромният брой останали GPU могат да бъдат утилизирани в трениране на дълбоки невронни мрежи. 

Ние сме развълнувани да работим върху нашата нова научна цел през 2018 г., тъй като тази година може да предостави уникална възможност за изграждане на първия децентрализиран суперкомпютър, отдаден за създаване на изкуствен интелект.

\section{Заключение} 

Блокчейн технологията дава възможност за нов тип търговия с криптоактиви, като по този начин се създават нови видове пазари и се разкриват множество нови приложения. Поради децентрализираната си и открита природа, блокчейнът предоставя изобилие от данни, които никога досега не са били на разположение. Достъпът до информация като баланса на всеки акаунт и всяка парична транзакция ни насърчава да търсим цялостен поглед върху динамиката на блокчейна.

В нашето проучваме ние сравнихме различни методи за изграждане на дълбоки невронни мрежи в способността им да намират коректни зависимости в блокчейн данните на Ethereum и да предоставят прогнози относно бъдещи черти на криптовалутата, включително цената на валутата. За да проведем експериментите си, ние създадохме рамка за събиране, обработка и съхранение на данни, която ни позволи да се справим с огромното количество данни от в блокчейна на Ethereum (повече от 1000GB) и ефективно да произвеждаме датасети за трениране.

Изпробвахме както рекурентни, така и конволюционни модели с различен датасет и цели на прогнозата. Най-интересните резултати идват от нашите конволюционни модели, които работят върху разпределителни хистограми на акаунти с едно, две и три измерения. Тези хистограми служат като ``картини'' на състоянието на блокчейна за определен период от време и когато наблюдаваме \href{youtu.be/czfBa75HuWs}{видео компилация от такива 2D хистограми}, ясно можем да видим тенденции, които са в съответствие с основните движения на пазара. След като експериментирахме с тези нови представителни данни за блокчейна, ние установихме, че конволюционните дълбоки невронни модели са в състояние да предоставят прогнози за стойността на валутата ETH, основаващи се единствено на данни от такива хистограми. Все пак смятаме, че по-добри резултати могат да бъдат постигнати чрез по-нататъшни оптимизации на ахритектурата и мета-параметрите. 

Понеже броят възможни комбинации за търсене на такива оптимизации е огромен, разработихме генетична рамка, която може да бъде използвана за генериране на оптимална невронна архитектура за определена прогнозна задача. Развълнувани сме от възможностите за автоматизиране на този процес. Нашата бъдеща работа ще бъде върху разработването и внедряването на децентрализирана мрежа от изчислителни системи, които предоставят изчислителната си мощ си на ``контролер'' алгоритми за генериране и оценяване на архитектури на дълбоки невронни мрежи.

\section{Благодарности}

Бихме искали да благодарим на г-н Божидар Маринов, в сътрудничество с когото разработихме генетичната рамка с отворен код, дефинирана в Раздел \ref{genetic-framework}. Бихме искали също така да благодарим на УчИМИ, за възможността да започнем проучването си на Лятната Изследователска Школа.

==> content/gsf_content_en.tex <==
\section{Summary}

\subsection{Project description (100w)}



\subsection{Project summary (250w)}

%why this
%problem and predicted outcome
%methodologies
%overview of the research
%application
%conclusion and why it supports hypothesis
%next steps

\section{Question / Proposal (250w)}

%main question
%specific, measurable question
%hypothesis
%expected outcome
%interpretation of results

The availability of computing power has allowed deep learning to thrive, with advancements in self-driving cars, translation, decease diagnosis, and computer vision just to name a few. However, neural networks have an undefined nature - it is difficult to guess which neural configuration will perform better on a specific task. Creating efficient neural networks often involves a continuous process of testing various hyperparameter and network topology configurations and the respective training and evaluation. Therefore, machine learning requires both deep expert knowledge and vast amounts of computing power, limiting the amount of problems that it can solve.

Recent advancements in the area explore the concept of Neural Architecture Search (NAS). These algorithms attempt to automate the process of deciding which modifications of the current neural configuration will lead to an increment in performance. This eliminates the human bottleneck in the process of creating neural networks.

We hypothesize that we can create such an algorithm in two ways - with a novel genetic approach, or by investigating and bettering the current state-of-the-art NAS paper. Performance will be measured based on the algorithm's ability to create efficient neural configurations for the problem of cryptocurrency predictions. This problem is chosen based on its difficulty and practical applications. It has been thoroughly explored in our previous research \cite{predictor}, which presents manually configured neural network configurations for the problem. We estimate that by developing an improved NAS algorithm for this specific task, it will also be applicable in other machine learning problems.


\subsection{Research}

%summary of work
%how this helps us
%how this research helps others

A set of recent publications on the topic of Neural Architecture Search have demonstrated different approaches which successfully beat state-of-the-art man-made models. Some of them include a Reinforcement Learning algorithm by Google \cite{google_nas}, a Differentiable Architecture Search approach by Deepmind \cite{deepmind_nas}, and a modified Bayesian optimization and Network morphism-based algorithm \cite{autokeras}. These papers demonstrate various successful approaches on automating neural architectures. Most of recent of those is the latter, which also presents an open source library called ``AutoKeras'' that implements their approach. This allows us to investigate this algorithm more closely, apply it for the problem of crypto predictions, as well as attempt modifications with the aims of improving it.

Bayesian optimization is widely used in problems that involve optimization of non-differentiable black-box functions. The algorithm analyzes the search space by making various observations of different parameter configurations. After an observation, it makes a guess where to probe next based on its previous observations. This allows it to both initially explore the diversity of the search space and later focus in the more promising areas once it identifies them. %background. maybe better suited for that section?

In June 2018 Jin, Song, and Hu introduced a paper on the topic of Efficient Neural Architecture Search with Network Morphism \cite{autokeras}. They propose an evolutionary NAS system that evolves a neural network configuration. The search space represents all neural network configurations, which is a tree space rather than a planar one. Bayesian optimization traditionally functions for planar fields and has hence been modified to explore the needed graph space.

The algorithm starts with a random neural configuration. Said network is trained and based on its accuracy an acquisition function proposes a morph (an observation) that will lead to an increment in performance. After every observation, the current network configuration is modified and only the new layers are retrained, hence reducing the training overhead.



When it comes to the specific predictive problem, notable work includes a paper by a Stanford University research group \cite{stanford-predictions} and two more recent github projects \cite{bitpredict} {\cite{deep-learning-bitcoin}}. All of which focus primarily on Bitcoin price estimations, do not explore the rich publicly available blockchain data in depth, and do not use or have not disclosed sophisticated deep learning techniques for their estimations.


\section{Test dataset}
\label{generated-datasets}

Our test data comprises of series of images, representing recent activity in the cryptocurrency Ethereum.

%IMAGE OF DISTRIBUTION HERE

This is an example image that represents the distribution of accounts on the base of their balance (Y axis) and time since last activity (X axis) on a log scale. The color scale represents a log of how many users fall within this spot in the intersection of the 2 distributions. More information on the dataset generation is defined in our research on cryptocurrency predictions \cite{predictor}.

\section{Genetic algorithm}
\label{nas}

Our first attempt towards creating a NAS algorithm is a genetic one that can create, support, and mutate a population of machine learning configurations, or solutions.

\begin{figure}
\centering\includegraphics[width=\graphwidth]{assets/genetic_engine}\hfill
\caption{Genetic algorithm scheme}
\label{genetic-framework-scheme}
\end{figure}

Solutions are encoded as a genome. Initially, we have a random population of genomes. They are converted to live deep networks, which receive a performance (fitness) score when evaluated. The next generation of genomes is created by mutating and mating the current population. The specific operations\cite{twopoint-crossover}\cite{uniform-crossover} are named in the algorithm flowchart. This process repeats in a loop.

\section{Improved NAS approach}

We are investigating the NAS approach by Jin, Song, and Hu \cite{autokeras} with the goal of improving its technical or theoretical setup. During initial experimentation with the algorithm, we have noticed the following problems and are proposing respective improvements to the authors' implementation:

\begin{itemize}
\item The acquisition function favors larger models which often do not fit within memory. There is no way for the algorithm to learn that a specific path is inefficient due to hardware constraints. Negative feedback should be given to a morph that surpasses hardware resources.

\item Not scalable on multiple GPUs. The approach is not a populational, but an evolutional one. Still, due to the sparsity of the search space, it might be feasible to run multiple evolutional paths in parallel. 

\item Data normalization is restricted to one method, which is mostly effective in image data. Additionally, the normalization state is calculated on the whole dataset, instead of only on the train subset. The latter may mitigate overfit. 

\item No support for cross validation. While it is a computationally heavy process, it is a good idea to periodically verify the performance of a specific network more objectively.

\item Only Dense and 2D Convolutional layers can be created. The algorithm does not support other types, such as recurrent layers. The technical implementation can be expanded to support them. This will allow the algorithm to be applied in more deep learning problems.

\item No regularization options, including L2 or Dropout. Regularization can be included as a possible morph type in order to reduce overfit.

\end{itemize}

So far we have improved the resource usage of the algorithm by penalizing it with negative feedback once it requests to create a model too large for the available system resources. This problem is the most severe of the aforementioned ones as often times the search process crashes due to insufficient system resources. Implementing said limits allows for the search to continue undertaking its optimization task.





\section{Experiments and results}
\label{experiments}

\subsection{Genetic algorithm}

%The expected prediction output is a boolean - whether the Ethereum price will fall or rise in the next hour.


The genetic algorithm experiment tries to create neural networks that emit ``buy'' and ``sell'' trade signals. Hence the performance metric is possible profits if we were to trade using these signals.

%took place before our work on the improved NAS approach and hence have a different performance metric - instead of measuring percentage of correctly predicted price changes, we measure possible profits if we were to trade listening to the predictions.

Running the genetic algorithm for a day has yielded a neural configuration that results in profits of $1.8$ times the initial investment in a simulated trading round between 15.09.2017 and 15.03.2018. The positive results from this experiment have motivated us to explore the problem in more depth and from a different angle.

\subsection{Improved NAS}

The experiments with the other NAS approaches took place after our genetic one and focus on creating networks that predict positive or negative price changes in the next hour.

\begin{table}
\centering
\begin{tabular}{l|l|l|l}
& Manual & Original NAS & Improved NAS \\\hline
Accuracy & 55\% & 70\% & 78\% \\
\end{tabular}

\caption{Highest accuracy of a network created by the different approaches}

\end{table}

The results shown are the highest performant networks created by three approaches - manually, via the default implementation of Jin, Song, and Hu \cite{autokeras}, as well as our improved NAS approach.

By trying to manually create the network, we achieved highest performance results of $55\%$ using the following Convolutional architecture and a year-long blockchain dataset.

\begin{figure}
\centering\includegraphics[width=\graphwidth]{assets/architectures_short_cnn}\hfill
\caption{A manually configured convolutional configuration}
\label{cnn}
\end{figure}


The most successful network created by the original NAS reaches 70\% classification accuracy on a week-long dataset. It must be noted that 70\% of the test labels in this case are 0, meaning that the algorithm was unable to find an efficient solution.

The improved NAS approach achieves a notable improvement with a 78\% classification score on the same dataset as the original.

The size of the dataset depends on how the network is generated. Because manually created networks are usually created once and expected to work for prolonged periods of time, our manual experiment uses a long dataset. However, with the flexibility of NAS algorithms, networks created by them only need to work in the short-term and then be replaced with an improved version. Hence the experiments with the NAS approaches utilize a smaller dataset. The NAS's better ability to generalize for the most recent short-term patterns may be one of the reasons why it achieves a significantly higher score than the manual approach.

A video illustration of the evolution of a neural architecture by the improved NAS can be \href{http://cli.re/gqKy9M}{seen here}.

The results look promising and demonstrate the need for further investigation in the topic.


\section{Conclusion}


%Blockchain technology enables a new class of tradeable cryptotoken assets, thus creating new kinds of markets and numerous new use cases. Due to their decentralized and open nature, public blockchains provide abundance of market-related data that has never been available before. Having every account balance and every transaction visible, encourages us to seek a holistic view on the blockchain dynamics.

BE CRITICAL HERE - WHAT ARE WE MISSING?

Our initial focus on the creation of a genetic algorithm for neural generation has lead to positive results. This indicates that such type of metaheuristics can be successfully utilized in neural generation problems and motivated us to explore other types of algorithms. Our later focus on improving the NAS approach by Jin, Song, and Hu \cite{autokeras} lead us to interesting discoveries about such NAS algorithms and uncovered a whole set of future development ideas that can be explored.

While we mainly emphasized on the problem of cryptoasset predictions as our experimental setup, it must be stated that these algorithms have potential applications in most areas where manually configured neural networks are currently being utilized.

Criticism can be made in regards to our choice of dataset. We have not disproven the case where the specific test samples used in the experiments are easier and hence not a reliable indicator of NAS performance. We need to repeat these experiments with multiple dataset configurations and search times to verify this.

Overall, our initial experiments have demonstrated promising accuracy reports and it is worth further investigating similar NAS approaches in the pursuit of creating an universal problem solver.


%When it comes to data, the most interesting results came from the account distribution histograms. These histograms serve as ``pictures'' of the blockchain in certain period of time and when we observe
%\if\showlinks1
%a \href{https://youtu.be/czfBa75HuWs}{time-lapse video of such 2D histograms (youtu.be/czfBa75HuWs)},
%\else
%their historical values,
%\fi we can clearly see patterns that correlate to major market moves.

\section{Acknowledgements}

We would like to thank Mr. Bojidar Marinov for the assistance in creating the genetic algorithm, Mr. Konstantin Delchev and Dr. Violeta Ivanova-Rohling for their expert guidance during the Summer Research School 2018, as well as HSSIMI for organizing said event.


==> content/nas_content_en.tex <==
\section{Introduction}

The availability of computing power has allowed deep learning to thrive to the point where neural networks are able to reach every industry. The advancements in self-driving cars, translation, decease diagnosis, and computer vision are only a few examples. However, it is difficult to guess which neural configuration will perform better on a specific task. Creating efficient neural networks often involves an endless process of attempting various hyperparameter and network architecture configurations. Most problems that require such complex tuning of neural configurations also demand for long training times. These factors make the process of neural optimization require both deep expert knowledge and vast amounts of computing power, limiting the amount of machine learning problems that can be solved.

Recent advancements in the area explore the concept of Neural Architecture Search (NAS). These algorithms attempt to automate the process of deciding which modifications of the current neural configuration will lead to an increment in performance. This eliminates the human bottleneck in the process of creating neural networks.

We would like to create an improved NAS algorithm. Its performance will be measured based on its ability to create efficient neural configurations for the problem of cryptocurrency predictions. This problem is chosen based on its difficulty and practical applications. It has been thoroughly explored in our previous research \cite{predictor}, which presents manually configured neural network models for the problem.

In Section \ref{background}, we introduce background information on Blockchain theory and Deep Learning. Section \ref{problem} defines the cryptoasset predictions problem and our test datasets. In Section \ref{experiments}, we compare our best manual results to a recently published NAS algorithm. Based on the experimental conclusions, in Section \ref{scynet}, we propose the creation of a new NAS algorithm, distributed in a blockchain. 

\subsection{Related work}

A set of recent publications on the topic of Neural Architecture Search have demonstrated different approaches which successfully beat state-of-the-art man-made models. Some of them include a Reinforcement Learning algorithm by Google \cite{google_nas}, a Differentiable Architecture Search approach by Deepmind \cite{deepmind_nas}, and a modified Bayesian optimization and Network morphism-based algorithm \cite{autokeras}. Out of these, we consider the latter as most interesting, as they also implemented their approach into an open source library called AutoKeras.

Multiple blockchain startups have also demonstrated interest in contributing to the machine learning field. OpenMined \cite{openmined} allows researchers to train their models on a private, distributed dataset, for example medical records, and SingularityNet \cite{singularity} allows modellers to sell their machine learning solutions as services. While these networks improve the machine learning work flow, they still require human intervention for the creation of the models in the first place.

When it comes to the specific predictive problem, notable work includes a paper by a Stanford University research group \cite{stanford-predictions} and two more recent Github projects \cite{bitpredict} {\cite{deep-learning-bitcoin}}. All of which focus primarily on Bitcoin price estimations, do not explore the rich publicly available blockchain data in depth, and do not use or have not disclosed sophisticated deep learning techniques for their estimations.


\section{Background}
\label{background}

\subsection{Blockchain and Ethereum}

%is this really needed?
Satoshi Nakamoto's introduction of Bitcoin in November 2008 \cite{bitcoin-paper} has often been hailed as a radical development in money and currency as it is the first example of a digital asset which simultaneously has no backing or ``intrinsic value'' and no centralized issuer or controller. Another arguably more important part of the Bitcoin experiment is the underlying blockchain technology as a tool of distributed consensus. The most important aspect of such technology is the absence of an intermediary (centralized server, bank, company, etc.) between the originator and the recipient, as any changes to the data on this chain are made by consensus among all members of a decentralized network. Thus, avoiding the need to trust third parties. The blockchain can be thought of as a distributed public database with records for each transaction in history. All cryptoasset operations and activity are contained within the blockchain transaction data.

The Ethereum project ($ETH$) is a newer implementation \cite{yellowpaper}, based on the blockchain technology. In addition to the transaction record keeping functionality, Ethereum provides a mechanism for executing program logic on each transaction through the concept of smart contacts. This significantly extends the use cases of blockchain technologies, reaching far beyond simple financial transactions - secure voting, autonomous organizations, company management, freedom of speech networks, online games, crowdfunding, speculation markets.


\subsection{Use of Deep Learning in asset value predictions}
Deep Learning \cite{deep_learning} allows for the discovery of patterns in a large dataset. Such a set consists of dataset samples (input-output pairs, such as summarized blockchain activity and the future price). The inputs pass through multiple layers (which perform data transformations with free parameters) and leave as an output. Deciding on an optimal arrangement, combination, and configuration of layers is the prime difficulty in creating deep networks. In order to evaluate a network, the free parameters of its layers have to be set (trained, learned) on known dataset input-output pairs.

Long Short-Term Memory (LSTM) \cite{LSTM} and Convolutional (CNN) \cite{cnn} networks are known types of DL networks, which are well known for their performance in time series and image analysis respectively.

\section{Blockchain predictions problem}
\label{problem}

The applications of Ethereum \cite{yellowpaper} make it one of the more noisy and difficult to predict blockchains. This is why we chose the problem of predicting Ethereum as the prime target for the evaluation of our neural networks.

The unprocessed blockchain data of Ethereum contains account balances and transactions. One of the more interesting ways to analyze that is to create two-dimensional account distributions, as seen in Figure \ref{balanceLastSeenDistributionExample}. These represent two crossed distributions - one of the cryptocurrency accounts by balance (horizontally), and one with the time since their last activity (vertically). Analysing a series of these distributions for different time periods, we can more effectively capture major market movements, as seen in a time-lapse video of these distributions (\href{https://youtu.be/Dwwnxn1j6AQ}{https://youtu.be/Dwwnxn1j6AQ}).

\begin{figure}[h]
\centering\includegraphics[width=0.8\graphwidth]{assets/distributions/balanceLastSeenDistribution_log1_2}
\caption{We observe the difference in activity of the most recently active accounts (left) and richest accounts (down). 
}
\label{balanceLastSeenDistributionExample}
\end{figure}

These observations motivated us to utilize a series of such distributions as the dataset inputs for our experiments. The expected output is a Boolean - whether the cryptoasset price will rise or fall within the next hour. Hence the performance metric of the algorithm is the percent of cases where it predics correctly. The baseline of a dataset is the maximum accuracy that can be achieved by predicting a constant value. %this can be explained better
This type of dataset is the basis of all experimental results.

The raw blockchain data we collect, the exact definition of the feature extraction algorithms, as well as the dataset shaping methodologies are defined in Appendices \ref{data-sources}, \ref{property-generation}, and \ref{dataset-generation} respectively.


\section{Manual deep network approach}

Our highest results on this problem using manually configured Neural configurations are achieved in our previous research \cite{predictor}. The successful configuration is a convolutional architecture, shown on Figure \ref{cnn}. Using a year-long dataset, the achieved results are a prediction sign accuracy of $55.12\%$ (50\% baseline) when trained on a year-long dataset.

\begin{figure}[h]
\centering\includegraphics[width=\graphwidth]{assets/architectures_short_cnn}\hfill
\caption{The manually configured convolutional configuration}
\label{cnn}
\end{figure}


\section{Neural Architecture Search approach}
\label{nas}

A possible method to find a more accurate neural configuration for this problem is Neural Architecture Search. The basic work flow of a NAS algorithm (Figure \ref{fig:nas}) is to continuously evaluate and modify a neural configuration to learn which type of modifications are best for the specific problem. 

\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{assets/NAS.png}
    \caption{High-level NAS operations}
    \label{fig:nas}
\end{figure}

The bigger challenge in the design of NAS algorithms is usually to define a modifier function that proposes architecture changes that effectively increase performance in later stages.

\texcomment{
\subsection{Genetic algorithm}

Our first attempt towards creating a NAS algorithm is a genetic one that can create, support, and mutate a population of machine learning configurations, or solutions.

A solution represents a specific deep network topology, layer configuration, and training parameters. This information is encoded in a genome, consisting of a set of chromosomes. Each chromosome represents an array of integers and has a specific type. Example types include input data configuration, training parameters and a deep network layer with its their parameters (ex. $Conv2d$, $LSTM$). We have created a $JSON$ specification that allows the notion of any deep network configuration, and a converter that creates said $JSON$ from a genome. The output $JSON$ is passed to a parser that creates and returns the deep model, ready for training. 

\begin{figure}
\centering\includegraphics[width=\graphwidth]{assets/genetic_engine}\hfill
\caption{Genetic algorithm scheme}
\label{genetic-framework-scheme}
\end{figure}

The flowchart of the genetic algorithm is shown in Figure \ref{genetic-framework-scheme}. Initially, a population of $n$ individuals (genomes) is created with random chromosomes that make up a valid configuration (ex. the size of a Deep layer cannot be negative or exceed the available system memory). The configurations are converted to the $JSON$ specification and parsed to deep models. If a configuration cannot be parsed due to being invalid, it is removed from the current population. The rest of the configurations are trained in a Reinforcement learning environment to emit ``buy'' and ``sell'' trade signals. Based on their performance on a validation set, the respective solutions are ranked with a fitness score. The next generation of solutions is created by mutating and mating the current population. The mutations are random and include bit flips in the chromosome values and removing or adding a chromozome. Pairs of configurations are selected via Fitness proportionate selection and Tournament selection and undergo Two-point crossover \cite{twopoint-crossover} and Uniform crossover \cite{uniform-crossover}. The top $x\%$ of performing individuals are not mutated, while the worst ones are removed to keep population numbers stable. The resulting configurations continue on to the next generation and the loop repeats until a good enough configuration is found.
}

\subsection{NAS using network morphism and bayesian optimization}

%Our early NAS experiments were done using a genetic algorithm that can create, evaluate, and mutate a population of machine learning solutions. While this served as a proof of concept, the achieved results were not satisfactory. 

In June 2018 Jin, Song, and Hu introduced a paper on the topic of Efficient Neural Architecture Search
with Network Morphism \cite{autokeras}. They define an evolutionary NAS technique that is based on a modified Bayesian black-box function optimization. The modifier function in their case is an acquisition function that learns which configuration areas in the search space are likely to increase performance. After every modification, only the changed layers are retrained, reducing training overhead.

We experimented with their technical implementation (AutoKeras library v0.2.3) and modified it to apply it for the prediction problem. % and discovered a significant setback. The acquisition function favors larger models which often do not fit within memory and there is no method that allows the algorithm to learn that certain paths in the search space are infeasible due to hardware constraints.

%We modified the algorithm by penalizing the acquisition function with negative feedback once it requests to create an oversized model. These constraints allow the search to continue undertaking its optimization task.



\section{Experiments and results}
\label{experiments}

We have conducted multiple experiments with the aforementioned NAS algorithm in different data setups. The most successful experiment so far includes the dataset, defined in Appendix \ref{generated-datasets}. Results are shown in Table \ref{tab:results}.

\begin{table}[h]
    \centering
    \begin{tabular}{c|c|c}
         & Manual & NAS \\\hline
        Accuracy & 55\% & 78\% \\\hline
        Baseline & 50\% & 70\% \\\hline
        Difference & 5\% & 8\% \\\hline
        Improvement & 10\% & 11.4\% \\\hline
    \end{tabular}
    \caption{Results}
    \label{tab:results}
\end{table}

It must be noted that the datasets used in the two experiments are of different length to reflect on the intended use case for both types of networks. Manual networks are expected to generalize for prolonged periods of time, which is why they were trained on a year-long dataset. NAS allows for the flexibility to find an efficient short-term solution from only the most recent data, which is why we focused on 7-day datasets. With that in mind, we can observe that the NAS results are on par with our best manually designed network. 

These results are consistent with the findings of several other researched NAS approaches, such as Google's reinforcement learning \cite{google_nas}, Deepmind's on Differentiable Architecture Search \cite{deepmind_nas}, and Jin, Song, and Hu's Bayesian optimization with network morphism \cite{autokeras}. All of these reach results similar or sometimes surpassing the best neural network models designed by humans.

The unanimous conclusion of all aforementioned researchers is that their results were achieved by utilizing large amounts of computational power. Further improvement of performance requires significantly more computational resources, which means that individual entities can hardly make progress and take full advantage of the potential NAS algorithms provide.



\input{content/scynet_spec.tex}





%\section{Future work}

%There are many problems and future development opportunities when it comes to the NAS algorithm, as has been outlined in Section \ref{contribution}. Hence, a significant portion of the future development will be to contribute to the open source algorithm.

%An alternative approach is to further develop our genetic algorithm. We have many proposals of how it could be bettered with more efficient mutations, selection operators, crossover conditions, as well as general population management. 

%It might be possible that the bottleneck to finding an optimal solution to the prediction problem is the quality of the data. In that case, if we do not see any noticeable performance improvements with the aforementioned plan, we will investigate better feature extraction algorithms and other blockchain technologies as a whole.

\section{ScyNet implementation}

Our plans are to use the presented blockchain protocol to implement a public blockchain network, which we will also call ``ScyNet''. 

%scynet is autonomous and scalable
Even with a small number of initially participating nodes, ScyNet can be a meaningful source of Machine Learning models that is entirely automated and autonomous. The only resource that this network requires to produce continuously improving models is computing power. 

%incentives & profit
Through the utility token economy and decentralized tournaments, the participating nodes in ScyNet earn, stake, and trade with native blockchain tokens, used also for the network's Proof-of-Stake consensus. As the economic utility of training Machine Learning agents is higher than that of mining hashes, it is reasonable to suggest that the market capitalization of the suggested network's utility token can be at least similar to the ones of the currently widespread Proof-of-Work networks.

If ScyNet is made operational, it can democratize the access to AI for many industries. Still, we see the most exciting early applications of the network in the algorithmic trading of crypto-assets. Thus, the network will have its economic incentives entirely within the blockchain domain. 

%ScyNet's domain problem will be the algorithmic trading of cryptoassets. It will be interesting to see how the results of the blockchain approach compare to our current ones from NAS and manual network tuning.


\section{Conclusion}

Our initial focus on the problem of blockchain analysis led to the manual creation of an effective neural network. We were surprised to see how applying the latest state of NAS research for this problem managed to create a neural network, reaching the same performance level, all without human intervention.

This experiment also demonstrated that the main constraint to what a NAS algorithm can achieve is the amount of computing power utilized. That motivated us to design a Blockchain protocol that incentivises independent computing nodes to execute NAS algorithms and compete in creating continuously improving solutions for a particular task. The nodes of the network can collaborate through an open market mechanism which allows for the stacking of different models that can provide even more informed predictions. 

Our future work will be towards providing a reference implementation of the presented blockchain protocol and establishing an operational network of computing nodes. 


%that allows domains to be easily created for various machine learning challenges. We are excited to see how this technology can impact research in the field and hope that it provides access to the latest state of ML algorithms to many smaller entities.

%This experiment also demonstrated that the  the reliance of common NAS algorithms to large computational resources, limiting who can create or use AI services. That motivated us to design a Blockchain protocol that incentivises independent computing nodes to execute NAS algorithms to compete by creating solutions to a given problem all while allowing external parties to access them.

%The protocol in its current state allows data analysts to sell their data, computer owners to provide ?, and is shown to be resistant against various theoretical attacks including the arbitrary failure of any of its member nodes. 

%When it comes to data, the most interesting results came from the account distribution histograms. These histograms serve as ``pictures'' of the blockchain in certain period of time and when we observe
%\if\showlinks1
%a \href{https://youtu.be/czfBa75HuWs}{time-lapse video of such 2D histograms (youtu.be/czfBa75HuWs)},
%\else
%their historical values,
%\fi we can clearly see patterns that correlate to major market moves.

%\section{Acknowledgements}

%We would like to thank Mr. Konstantin Delchev and Dr. Violeta Ivanova-Rohling for their expert guidance during the Summer Research School 2018, as well as HSSIMI for organizing said event.


%temp positioning
\bibliographystyle{agsm}
\bibliography{references}


\newpage


\appendix
\section{Raw blockchain data}
\label{data-sources}

The first kind of data gathered is historical market tick data, which is aggregated from multiple exchanges to achieve a less biased view of the financial state. The frequency (size of each market tick) is one hour. Every tick consists of the $open$, $close$, $low$, and $high$ prices, as well as the trade volume to and from the currency for that period. 

The second kind of data is from the Ethereum blockchain. It grows every day \cite{blockchain-size} and includes hundreds of gigabytes worth of transactions, cryptocontract executions, and blockchain events for every moment its existence. For each block in the chain, the following data points are extracted: creation timestamp, number (chain index), miner (block creator), list of confirmed transactions, size in bytes, creation difficulty, and computational resources used (Gas limit and Gas used). The following is stored for each transaction in a block: address of the initiator and receiver, transferred value, used resource units (Gas), and amount paid per resource unit (Gas price). The same kind of information is also collected for internal contract activity by calculating transaction traces.

The total size of the gathered raw blockchain features is around 500GB, containing $5,300,000$ blocks with a total of $194,000,000$ transactions and close to a billion traces. It took 30 consecutive days to download and another 14 to process, filter, format, and save the data to a database.

Both the market and blockchain data are collected for the interval from 8-08-2015 to present.

\section{Generation of data properties}
\label{property-generation}

In order to create a blockchain-based dataset, we first need to extract more valuable information from the raw blockchain data by defining  feature extraction algorithms. A feature (also called property) is calculated once for each market tick in the historical data in order to form a time series.

More specifically, we are investigating methods to track the activity of cryptocurrency accounts in higher detail. This is achieved by creating account distributions - 2D matrices that visualize account activity based on multiple account features. These distributions contain spatial value, which Convolutional networks can take advantage of. 

Let us introduce some common definitions: $scl$ as an array of scale functions, $feat$ as an array of functions that return an account feature, and $mx$ as an array of constants.

Possible values for $scl_i$ include $\log_2$ and $\log_{1.2}$. Possible account features ($feat_i$) are defined in Table \ref{account_feature_table}.

\begin{table}[h]
\centering
\begin{tabular}{lp{6cm}}
Feature & Description \\\hline
balance & Account balance, measured in $wei$ ($10^{18}$ $wei$ = 1 $ETH$). \\
lastSeen & Amount of seconds since the account's last participation in a transaction. \\
volumeIn & Amount of received value in the last tick, in $wei$. \\
volumeOut & Amount of sent value in the last tick, in $wei$. \\
transactionN & Amount of transactions where the account is either a receiver or a sender.\\
ERC20 & Amount of ERC20 token operations in the last tick (Ethereum contracts only) \\
\end{tabular}
\caption{\label{account_feature_table}The possible account feature functions.}
\end{table}

\subsection{Account balance distribution}
\label{account_balance_distribution}

This distribution visualizes summarized recent account activity in terms of the exchanged volume and amount of transactions, distributed based on balance groups.

Let us define $scl_0 = \log_2; \; mx_0=10^{26}; \; feat_0=volumeIn; \; feat_1=volumeOut; \; feat_2=transactionN; \; groupN = \lfloor\ scl_0(mx_0)\rfloor; \; featN=3$, $S$ as the accounts that have participated in a transaction throughout the current market tick, and $distribution$ as a matrix of shape $(featN, groupN)$.

\vspace{4em} %tmp

For $acc \in S$:

\hspace{3em} $gr = \min(\lfloor scl_0(balance(acc))\rfloor, groupN-1)$

\hspace{3em} For $x \in [0, featN)$:

\hspace{6em} $distribution_{x, gr} \; += feat_x(acc)$

$distribution = scl_0(distribution)$

The final operation is to scale the large values of volumeIn and volumeOut.

Figure \ref{account_balance_graph} contains an example of $2$ such distributions.

\begin{figure}[h]
\centering\includegraphics[width=\graphwidth]{assets/distributions/accountBalanceDistribution_log1_2}\\
\centering\includegraphics[width=\graphwidth]{assets/distributions/accountBalanceDistribution_log2}
\caption{Examples with $scl_0=\log_{1.2}$ (up) and $scl_0=\log_{2}$ (down). We observe how the summarized account trade activity changes in the different balance groups.}
\label{account_balance_graph}
\end{figure}

\subsection{Account number distributions}
\label{account_number_distribution}

These multivariate distributions represent how the accounts are clustered based on 2 of their account features.

The process of creating an account number distribution is described as follows:
\vspace{1em}

Repeat for $x = 1$ and $x = 2$:

\hspace{3em} $groupN_{x} = \lfloor scl_{x}(mx_{x})\rfloor$

For $acc \in S$, where $S$ is a chosen subset of (or all) accounts, do:

\hspace{3em} Repeat for $x = 1$ and $x = 2$:

\hspace{6em} $group_{x} = \min(\lfloor scl_{x}(feat_{x}(acc))\rfloor, groupN_{x}-1)$

\hspace{3em} $distribution[group_1, \; group_2] \; += 1$

Finally, for every value, do:

\hspace{3em} $distribution = \log_2(distribution)$

The final $\log_2$ scaling is to mitigate the uneven distribution of accounts. Some configurations of this type of distributions are presented in Table \ref{account_number_table}.

\begin{table}[h]
\centering
\setlength\tabcolsep{1.5pt} % TEMPORARY FIX
\begin{tabular}{lrrrrrrrp{5cm}}
$N$ & $S$ & $feat_1$ & $feat_2$ & $scl_1$ & $scl_2$ & $mx_1$ & $mx_2$ \\\hline
1 & all & balance & lastSeen & $\log_{1.2}(\lfloor x / 10^{17} \rfloor)$ & $\log_{1.2}$ & $10^{7}$ & $20736e3$ \\
2 & contracts & balance & lastSeen & $\log_{1.2}(\lfloor x / 10^{17} \rfloor)$ & $\log_{1.2}$ & $10^{7}$ & $20736e3$ \\
3 & contracts & volumeIn & ERC20 &  $\log_{2}(\lfloor x / 10^{17} \rfloor)$ & $\log_{2}$ & $10^{7}$ & $262144$ \\
\end{tabular}
\caption{\label{account_number_table}The configurations for account number distributions. The balances and transfers, measured in wei, are scaled to larger units ($10^{17}$ $wei$ = $0.1$ $eth$) to reduce noise.}
\end{table}

Consequently, we refer to the distribution configurations as follows: balanceLastSeenDistribution (N=1), contractBalanceLastSeenDistribution (N=2), and contractVolumeInERC20Distribution (N=3). Example distributions are visualized in Figure \ref{account_number_example}.

\begin{figure}[h]
\centering\includegraphics[width=0.8\graphwidth]{assets/distributions/balanceLastSeenDistribution_log1_2}\\
\centering\includegraphics[width=0.7\graphwidth]{assets/distributions/contractVolumeInERC20Distribution_log2_v2_stateless}
\caption{
\textbf{balanceLastSeenDistribution (up)}: we observe the difference in activity of the most active accounts (left) and richest accounts (down). The empty lines are seen because $\lfloor\log_{1.2}(x)\rfloor \notin \{1, 2, 4, 5\}$ for all $x$.
\if\showlinks1
User behavior and major market movements are more effectively seen in a time-lapse video of the distribution values (\href{https://youtu.be/Dwwnxn1j6AQ}{https://youtu.be/Dwwnxn1j6AQ}).
\fi
\\\textbf{contractVolumeInERC20Distribution (down)}: we observe the correlation of a crypto contract being used ($X$) and the amount of funds received from it ($Y$).
}
\label{account_number_example}
\end{figure}

\section{Generation of a dataset}
\label{dataset-generation}

A dataset is a set of samples, containing inputs (normalized property data) and expected outputs (prediction target). The concepts and methodologies behind dataset generation are defined in the following subsections.

\subsection{Prediction target}
%not sure if 51% attacks should be mentioned
The prediction target is the future value a chosen target property. Predictions are for the duration of one market tick. Examples of a prediction target include relative price fluctuations, amount of new accounts, trade volume, transaction count, and network stagnation (which has been a considerable issue in the past \cite{blockchain-clogging}).

Our experiments are be mainly focused on predicting price movements.

\subsection{Normalization}
\label{normalization}

Let us define the following normalization algorithms:

$$basic_i = \frac{x_i - min(x)}{(max(x) - min(x))}$$

This basic min-max scale is used to map independent sequences with the same sign to the interval $\in [0; 1]$.

$$around\_zero_i = \frac{x_i + max(\lvert max(x) \rvert, \lvert min(x) \rvert)}{2*max(\lvert max(x) \rvert, \lvert min(x) \rvert)}$$

Similar to $basic$, but maps positive and negative inputs to $(0.5; 1]$ and $[0; 0.5)$ respectively. This scale is used with sequences of varying sign.

%do I need to specify what is std?
$$image_i = (x_i - \frac{1}{n}\sum_{t=1}^{n}x_t) * \frac{1}{std(x)}$$

An an algorithm which produces unbounded time series of zero mean and equal variance. It is used with image-line sequences.

Every property in a dataset is a different time series and is normalized separately with a chosen algorithm. A method to automatically determine the algorithm for a given property is called $prop$, which uses $basic$ scale if the property values are absolute and $around\_zero$ scale otherwise.

Most of the algorithms scale on the basis of $\min$ and $\max$ bounds, hence future values may not fit that initial scale. The problem is mitigated if the normalized values are relative, which has also resulted in lower overfit and higher prediction accuracy in our experiments.
%the below technique is not used
%We also use a technique called normalization space overprovisioning, which increases the initial $\min$ and $\max$ values by a given percentage so that future values are more likely to fit.
%The problem of future values can be solved completely by using $local$ normalization, but that is not the best algorithm in all cases.
%All of the aforementioned methods to deal with the problem can be used in conjunction with each other.





\subsection{Dataset models}
\label{dataset-models}
The dataset samples (input-output pairs) are created using a sliding window with a size of $wn$ and step increments of $1$ over a chosen set of normalized property values. Let us define a property's values as $prop_y$, where $y < propN$, a specific value in a property time series as $prop_{y,x}$, and $prop_{t}$ as the prediction target.

$step=0$

For $x \in [0, wn-1]$, do:

\hspace{3em} For $y \in [0, propN-1]$, do:

\hspace{6em} $win_{x,y} = prop_{y,x+step}$

\hspace{0em} $tar = prop_{t, wn+step}$

Where $win$ is the window (unstructured dataset input), $tar$ is the expected output, and $step$ is incremented for each window.

In order to combine multiple normalized properties in a single dataset, we need the following model that defines how their values are arranged in N-dimensional space.


\subsubsection{Stacked layers model}
\label{stacked-model}

%\begin{wrapfigure}{R}{0.5\graphwidth}
\begin{figure}
%\centering\includegraphics[width=\linewidth]{assets/stacked_model}
\centering\includegraphics[width=0.5\graphwidth]{assets/stacked_model}
\caption{Visualized sample of the stacked layers model, where $wn=3$ and the chosen properties consist of balanceLastSeenDistribution.}
\label{stacked_model_example}
\vspace{-0pt} %workaround, because wrapfigure hates the float package
%\end{wrapfigure}
\end{figure}

A given set of property values (a column in $win$) has shape $(v_1, v_2, wn)$, where $v_1 = 1$ and $v_2 = 1$ for all properties but the distributions (discussed in Sections \ref{account_balance_distribution} and \ref{account_number_distribution}). The stacked layers model is a 3D structure that matches input shape for the Convolutional Neural Network and allows modeling of 3D shaped property windows, preserving their spatial value. 

The model defines a 3D matrix $mat$ of shape $(values_1, values_2, wn)$. A dataset sample $mat$ is created as follows. For every set of windowed property values $vals$:

$$mat_{s_1 + (0 \; to \; v_1), s_2 + (0 \; to  \; v_2), 0 \; to \; wn} = vals_{0 \; to \; v_1, 0 \; to \; v_2, 0 \; to \; wn}$$

Where $s_1$ and $s_2$ are set to the smallest integers where no values of other previously assigned properties are overridden. A visualized sample produced this model is seen in Figure \ref{stacked_model_example}.

\vspace{1pt} %to move the title of the next section to the next page



\section{Generated datasets}
\label{generated-datasets}

Our NAS experiment includes one variant of a dataset configuration. It comprises of the property $balanceLastSeenDistribution$ using the stacked model with $24$ $window\_size$ and $image$ normalization. The dataset spans 10 days after \textbf{2017-09-07}, where the train dataset is the first 7 days and the network performance is evaluated on the last 3. The expected neural network output is a classification on whether $highPrice$ increases or falls in the next tick.

In our prevoius experiments \cite{predictor}, datasets covering huge time intervals have consistently demonstrated lower performance on recent data. Cryptoassets are very volatile and we are only interested in analyzing the latest market trends, contained in the activity of the last couple of days. This short-term approach would only be practical with automatically generated neural networks, as a new configuration needs to be created for every new market trend.


\if\showlinks1
\section{Blockchain analysis framework}

The technical implementation for the blockchain problem, including data processing, dataset generation, and manual neural network definitions, is developed into an open MIT-licensed Blockchain analysis framework. The framework allows for the prediction of a chosen cryptocurrency on the basis of user-defined property extraction and neural algorithms. \href{https://github.com/Zvezdin/blockchain-predictor}{The GitHub repository of the project can be found at: https://github.com/Zvezdin/blockchain-predictor}

%The repository includes technical documentation, such as setup and usage instructions, so that others can both replicate our results and improve upon them.

%The Wiki about the project, including additional information for the research, \href{https://github.com/Zvezdin/blockchain-predictor/wiki}{is available here: github.com/Zvezdin/blockchain-predictor/wiki}

%The genetic algorithm and available under \href{https://github.com/obecto/gattakka}{the following address: https://github.com/obecto/gattakka}

%The improved NAS implementation requires more work until it is in a state where others can contribute to it or utilize it in their problems. We will publish the source code when that happens.

\fi

\section{Formal ScyNet protocol definition}
\label{formal-scynet}

All of the roles and functions of the proposed blockchain network can be more formally represented through the ScyNet blockchain protocol. It represents a set of transactions and a consensus mechanism that build an independent blockchain for the creation, verification, and utilization of machine learning agents.


\subsection{Underlying blockchain}

On a lower level, a ScyNet domain builds an independent blockchain network and a blockchain structure. The network behaves similarly to Bitcoin \cite{bitcoin-paper}, where any external node can connect with other peers, synchronize the blockchain, interact with the network by signing transactions, as well as participate in the consensus by verifying transactions and blocks.

\subsubsection{Domain token}

Every domain network creates a non-mintable token of a fixed supply. This token is used in all network payments to incentivise the consensus and commitments of the three types of hatcheries - harvesters, miners, and clients.

\subsubsection{Consensus}
\label{consensus}

Bitcoin's consensus relies on the GPU-heavy Proof-of-Work mechanism, known as ``mining''.
%The first version of the ScyNet protocol includes a placeholder Proof-of-Authority consensus which will be replaced with the Proof-of-Stake variant called ``Coin Age based selection'' after the finalization of the core ScyNet functionality.
ScyNet domains use a more efficient consensus mechanism in order to utilize GPU power for useful work. The consensus is a variant of Proof-of-Stake \cite{PoS} called ``Coin Age based selection'', as introduced in the PeerCoin cryptocurrency \cite{coin-age-selection}. The consensus power (probability for a specific node to win a block) is proportional to the number of cryptocurrency tokens the node has ``staked'', multiplied by the amount of days since it staked them. The timer is reset every time a node changes its stake or wins a block. This mechanism makes block creation more evenly distributed among the competing nodes, because the timing mechanism allows nodes with smaller amounts of stake to have a significant chance at winning a block overtime. %The exact specifics of the consensus will be defined in our testnet launch. %FIX THIS statement if it requires fixing?

\subsubsection{State replication}

A ScyNet domain network is built with the Tendermint framework \cite{tendermint}. It allows for the secure and consistent replication of a state machine (application) over many computing nodes. This means that once we define the types of transactions and the respective logic for their handling, Tendermint can consistently propagate these transactions through our peer network so that every node is on the same application state after every transaction. The framework is also Byzantine fault tolerant as it can tolerate the arbitrary failure of up to $\frac{1}{3}$ of the participating peers.

A network based on Tendermint works as follows. First, nodes submit transactions that reach every other node in the P2P network and enter the nodes' $mempool$. Upon a configurable event, a distributed pseudo-random function is executed that selects one node on the base of its consensus power. This node selects transactions from the $mempool$, creates a block, and submits it to the network. The block has to be signed by nodes with at least $\frac{2}{3}$ of the network's total consensus power in order for it to be accepted on the blockchain. If this step fails within a timeout, a new block creator is selected. 


\subsection{Domain configuration}
\label{domain_config}

The definition of a domain network includes setting a few specific parameters. This defines the tournament schedule and validation parameters, which depend on the specific machine learning problem being solved:


\begin{itemize}
    \item tournamentStartFrequency (Integer, milliseconds) - A tournament will start every x milliseconds, measured from UNIX Epoch. The tournament ends right before the start of the next one;
    \item proposerDeadline (Integer, milliseconds) - Period after the tournament where a selected proposer node must submit a tournament ranking;
    \item timeTolerance (Integer, milliseconds) - Latency tolerance for timed transactions;
    \item problemType (``real-time'' or ``dataset'') - Type of machine learning problem;
    \item realTimeFrequency (Integer, milliseconds) - For real-time problems, a real-time tick is defined as every x milliseconds, measured from UNIX Epoch;
    \item datasetSubmissionDeadline (Integer, milliseconds) -Deadline for challengers to submit dataset inputs after tournament start;
    \item minAgentChallengers (Integer) - Minimum number of nodes that have to independently challenge a submitted agent;
    \item minAgentChallengerVotingPower (Percentage) - Minimum share of the network voting power that has to challenge a submitted agent;
    \item agentSubmissionFee (Domain tokens) - Fee for a miner to submit an agent for a tournament;
    \item dataPublishFee (Domain tokens) - Fee for a harvester to publish a data offering;
    \item pricePublishFee (Domain tokens) - Fee for a miner to advertise his agent on the chain;
    \item rentFee (Domain tokens) - Fee withdrawn when a client rents an agent.
\end{itemize}

Outside the blockchain consensus, every domain needs a technical implementation of the blockchain node that defines all off-chain specifics, such as data formats, which error function is used in agent evaluation, or what external data do the nodes need to evaluate agents. Other responsibilities of the node implementation are discussed in Section \ref{node-functionality}.

\subsection{Node responsibilities}

The high-level overview (Section \ref{scynet}) presented the main roles and responsibilities and this section defines the specific protocol that every network node must follow to achieve that. References will be made to both the domain configuration (Section \ref{domain_config}) and the different network transactions (Section \ref{transactions}).


\subsubsection{Harvester actions}

In order for a hatchery to provide a data stream (real-time or of specific quantity) and advertise it on the blockchain, it must:

\begin{enumerate}

\item Submit publish\_data\_price transaction (Section \ref{publish_data_price}), paying the $dataPublishFee$;

\item Listen for rent transactions \ref{rent} that are directed to the harvester;

\item Communicate with the sender off-chain and privately give access to the requested quantity or duration of data.

\end{enumerate}


\subsubsection{Miner actions}

In order to verify and sell an agent on the network, a miner should:

\begin{enumerate}
    \item Send submit\_agent transaction (\ref{submit_agent}), paying the \mathbreak$agentPublishFee$;
    \item If domain is real-time:
    
    \begin{enumerate}
        \item Wait for the first real-time tick after tournament start;
        \item Generate an AES-256 key, generate an agent signal, encrypt the signal, and send submit\_signal transaction (\ref{submit_signal});
        \item At the next real-time tick, reveal the decryption key with publish\_signal\_decryption\_key transaction (\ref{publish_signal_decryption_key});
        \item Repeat from $b$ for every real-time tick until tournament end.
    \end{enumerate}
    
    \item If domain is dataset:
    
    \begin{enumerate}
        \item Wait for consensus to select the tournament challengers and then listen for publish\_dataset transactions (\ref{publish_dataset}) from the challengers until the \mathbreak$datasetSubmissionDeadline$;
        \item Download the datasets, generate all agent signals, generate an AES-256 key, encrypt the signals, and send submit\_signal transaction (\ref{submit_signal});
        \item Wait for tournament end and reveal the decryption key with publish\_signal\_decryption\_key transaction (\ref{publish_signal_decryption_key}).
    \end{enumerate}
    
    \item If the miner decides, it may submit publish\_agent\_price transaction \ref{publish_agent_price} to advertise his agent as a service;
    \item Listen for rent transactions \ref{rent} that are directed to the miner;
    \item Communicate with the sender off-chain and privately give access to the requested agent use.

\end{enumerate}

Failing to submit all required signals by the domain type will render the miner as disqualified from the tournament.

\subsubsection{Challenger actions (dataset domains)}
\label{challenger-actions}

The discussed consensus algorithm in Section (\ref{consensus}) presented a method to pseudo-randomly select one node from the network for block creation. The same algorithm is also used to select tournament challengers with the following additional rules:

\begin{enumerate}
    \item The selection process starts at tournament start;
    \item A miner, participating in the tournament, cannot be selected;
    \item There must be at least $minAgentChallengers$ challengers selected;
    \item The total consensus power of selected challengers must be at least $minAgentChallengerVotingPower$;
    \item There cannot be a challenger that comprises more than 10\% of the total challenger consensus power;
    \item Run the selection algorithm until these conditions are met.
\end{enumerate}


Once selected, every challenger must:

\begin{enumerate}
    \item Run a domain-specific algorithm to generate a validation dataset.;
    \item Generate an AES-256 key, encrypt the dataset outputs, and submit the dataset through the publish\_dataset transaction(\ref{publish_dataset}) by the $datasetSubmissionDeadline$;
    \item Wait for tournament end and submit dataset outputs decryption key via publish\_dataset\_decryption\_key (\ref{publish_dataset_decryption_key}).
\end{enumerate}


Failing to follow these rules by either not submitting a required transaction by the deadline, or submitting an invalid one, will result in the specific challenger being marked as disqualified, losing this role for the present tournament.


\subsubsection{Common actions for every node}

\begin{enumerate}
    \item If domain is real-time:
    
    \begin{enumerate}
        \item Listen for submit\_signal transactions (\ref{submit_signal}) from the miners;
        \item Listen for publish\_signal\_decryption\_key transactions (\ref{publish_signal_decryption_key});
        \item Wait for tournament end and decrypt all received signals;
        \item Make a local ranking of agents based on their prediction accuracy.
    \end{enumerate}
    
    \item If domain is dataset:
    
    \begin{enumerate}
        \item Listen for publish\_dataset transactions (\ref{publish_dataset}) from the challengers;
        \item Listen for submit\_signal transactions (\ref{submit_signal}) from the miners;
        \item Listen for publish\_dataset\_decryption\_key (\ref{publish_dataset_decryption_key}) from the other challengers;
        \item Listen for publish\_signal\_decryption\_key transactions (\ref{publish_signal_decryption_key}) from the miners;
        \item Decrypt all received signals and make a local ranking of the agents based on their average score among all challenger datasets;
        \item If any challenger misbehaves, mark him internally as disqualified.
    \end{enumerate}
    \item If any miner misbehaves, mark him as disqualified as well.
\end{enumerate}

A misbehaving node is one that did not follow the protocol of its role and either did not submit a required transaction, or submitted an invalid one. If a node marks another as disqualified, this is only internally known by the node itself. 

The first block creator that is selected after a the $proposerDeadline$ must include its local tournament ranking in the block by including the publish\_tournament\_ranking (\ref{publish_tournament_ranking}) transaction. This transaction will grant the tournament reward according to the rules in Section \ref{tournament_reward}. If another node receives a block after the specific deadline, the tournament results have not already been written to the blockchain, and a valid publish\_tournament\_ranking (\ref{publish_tournament_ranking}) transaction is not present, the block must be rejected. When a block is rejected, the consensus selects a new block creator who will, in this case, also be obliged to submit the ranking.

If the block creator has internally disqualified challengers with $\geq 50\%$ of the consensus power of all challengers, the tournament is considered a failure. In this case, the tournament\_failure (\ref{tournament_failure}) transaction has to be submitted instead, refunding all received fees that comprise the failed tournament reward.

\subsubsection{Tournament reward}
\label{tournament_reward}

All $agentSubmissionFee$ and \mathbreak$dataPublishFee$, and $rentFee$ received before the start of a tournament comprise the tournament reward. When a valid \mathbreak publish\_tournament\_ranking (\ref{publish_tournament_ranking}) transaction is received, the balance of the reward is granted by the following principles:

%placeholder numbers
\begin{itemize}
    \item If the domain is real-time, award the non-disqualified miners behind the top 3 performing agents in ratio 3:2:1;
    \item If the domain is dataset, the first $\frac{1}{3}$ of the reward is assigned to the non-disqualified challengers in ratio of their consensus power. The rest is assigned to the non-disqualified miners behind the top 3 performing agents in ratio 3:2:1;
    \item If $\leq 3$ and $\geq 1$ agents are from non-disqualified miners, the reward is split on 3:2 or 1 ratio;
    \item If 0 agents have survived, the reward is transferred to the fund of the next tournament.
\end{itemize}







%old, voting
%After tournament validation has passed:

%\begin{enumerate}
%    \item If the positive votes are >50\% of the total validator voting power at tournament start, validator consensus is reached and the tournament reward is released.
%    \item If the negative votes surpass the same margin, it is considered that the proposer falsified the ranking. The proposer is disqualified, a new one is selected among the remaining non-disqualified validators. The proposer sends a new ranking and the voting is restarted. 
%    \item If neither votes are enough for a simple majority, the tournament is considered a failure. All paid fees for this tournament reward are transferred to the next one and the competing agents receive the right to participate in the next tournament for free.
%\end{enumerate}

\subsection{Transaction types}
\label{transactions}

All blockchain communication in a domain is executed through transactions. Every hatchery holds an identity (account) on the network and should sign any outcoming transactions with it. An incorrectly signed transaction is invalid. Invalid transactions will be rejected by any peers and will not be propagated through the network or included in a block.

In the following subsections we describe in detail every type of transaction with its arguments, effect, and validity.

\subsubsection{submit\_agent($UUID$)}
\label{submit_agent}

Sent by a miner hatchery to notify that it has an agent that it wants to verify in the next tournament. Transaction arguments include an $UUID$ by which this agent will be identified in future communication. Sending this transaction will automatically withdraw $agentSubmissionFee$ amount of tokens from the miner's balance.

The transaction is invalid if the proposed $UUID$ is already taken by another agent, or if the miner does not have enough tokens to pay the fee.


\subsubsection{publish\_dataset($inputsURL$, $inputsHash$, \mathbreak$encryptedSignalsURL$, $signalsHash$)}
\label{publish_dataset}

Only exists in dataset domains. It is used by tournament challengers to publish the inputs of their personal dataset (accessible through $inputsURL$) so that competing miners can prove their agents' performance on it. The challenger generates a random AES-256 key and encrypts and uploads the correct dataset outputs (through $encryptedSignalsURL$). Hashes of the inputs and decrypted outputs are provided for future verification. 

The transaction is invalid if it is not signed by a selected tournament challenger, if the same challenger already submitted a transaction of this type during the same tournament, or if the $datasetSubmissionDeadline$ of the current tournament has passed.


\subsubsection{submit\_signal($agentUUID$, $encryptedSignal$)}
\label{submit_signal}

Sent by a miner hatchery to submit an AES-256 $encryptedSignal$ from a specific agent ($agentUUID$). Every signal must be encrypted with a different, unique, AES key.

The transaction is valid if $agentUUID$ exists and is claimed by the signing miner through a previous submit\_agent.

Additionally, if the problem is real-time, the transaction is valid only if received within a $timeTolerance$ of the specific real-time tick. It is invalid if the same transaction type has already been sent by the same miner and with the same $agentUUID$ for the same tick. If valid signal transactions for all ticks throughout a tournament are not received, the miner is disqualified.

If the problem is $dataset$, the transaction is valid only if received during an active tournament. It is invalid if the same transaction type has already been sent for the same $agentUUID$. If not received, the miner is disqualified from this tournament.

\subsubsection{publish\_dataset\_decryption\_key($key$)}
\label{publish_dataset_decryption_key}

Only exists in dataset domains. Every tournament challenger has to send this after the end of a tournament and reveal the encryption key that was used to encrypt the correct dataset outputs in publish\_dataset. 

The transaction is invalid if not signed by a non-disqualified tournament challenger, not received within a $timeTolerance$ of the tournament end, or the same transaction type has already been sent by the same challenger after the end of the same tournament.

If a tournament challenger does not submit this valid transaction, he is disqualified.

\subsubsection{publish\_signal\_decryption\_key($agentUUID$, $key$)}
\label{publish_signal_decryption_key}

Sent by a miner a specific amount of time after signing submit\_signal to reveal the AES-256 key by which the original signal was encrypted. 

The transaction is valid if $agentUUID$ is a previously registered agent by the signing non-disqualified miner and $key$ has not been previously used in this tournament.

If the problem is real-time, the transaction is only valid if received within a $timeTolerance$ of a specific real-time tick and $key$ successfully decrypts the signal received in submit\_signal transaction for $agentUUID$ from the previous real-time tick.

If the problem is dataset, the transaction is only valid if received within a $timeTolerance$ of the tournament end and $key$ decrypts the previously submitted signal. %potential problem - too large outputs mean slow TX verification.

If the signal is for an agent competing in an active tournament and a valid key is not received by the end deadline, the miner who owns the agent is disqualified.

\subsubsection{publish\_tournament\_ranking($ranking$)}
\label{publish_tournament_ranking}

Writes the results of a successful tournament on the blockchain - a ranking of the competing non-disqualified agents and their respective performance scores. Upon receiving a valid transaction, the node must update its state to grant the tournament award in accordance to Section \ref{tournament_reward}.

Transaction is only valid if:

\begin{itemize}
    \item The signer is the block creator;
    \item The transaction is received after a tournament end (and preferably but not enforceably before the $proposerDeadline$);
    \item The tournament is successful;
    \item The ranking exactly matches the node's internal ranking;
    \item The ranking for this tournament has not been successfully submitted already.
\end{itemize}

\subsubsection{tournament\_failure}
\label{tournament_failure}

Sent to notify for a failed tournament. Upon receiving a valid transaction, the node must update its state to refund all $agentSubmissionFee$ or $dataPublishFee$ that were received for the failed tournament's reward.

Transaction is only valid if:

\begin{itemize}
    \item The signer is the block creator;
    \item The transaction is received after a tournament end (and preferably but not enforceably before the $proposerDeadline$);
    \item This transaction has not already been submitted for the same tournament.
\end{itemize}


%\subsubsection{vote\_tournament\_ranking($vote$)}
%\label{vote_tournament_ranking}

%The other tournament validators cast votes (``for'' or ``against'') the proposed tournament ranking.

%Transaction is valid if the signer is a selected non-disqualified tournament validator, the transaction is received by the end of tournament validation, and the validator has not voted already in this tournament.

%A tournament validator which does not submit a valid transaction by the deadline will be disqualified.

\subsubsection{publish\_agent\_price($agentUUID$, $scheme$, $price$)}
\label{publish_agent_price}

A miner can allow his agent to be rented, or subscribed to, by other hatcheries. There are two types of payment schemes - paying the $price$ for every time you use an agent, subscribing to the agent and being able to use it for a specific period, or directly buying the algorithm. This transaction withdraws $pricePublishFee$ from the miner's account.

The transaction is valid if the signer has previously successfully had $agentUUID$ validated in a tournament, or if the signer does not have balance for the fee.


\subsubsection{publish\_data\_price($dataUUID$, $dataParams$, $scheme$, $price$)}
\label{publish_data_price}

A harvester can freely publicize what data it intends to sell to miners for the training of their agents. Details, including the shape, frequency, and further description of the data features are included in $dataParams$, which is a domain-specific data structure. The $scheme$ and $price$ parameters have the same functionality as in publish\_agent\_price. Submitting this transaction will withdraw $dataPublishFee$ domain tokens from the harvester's account.

The transaction is valid if the signer has enough balance to pay the fee and $dataUUID$ has not been previously assigned to an agent or data provider.

\subsubsection{rent($UUID$, $quantity$)}
\label{rent}
%possible problem - spam if miner agrees to set really low price. Can be resolved if the DAO imposes a fee on all rents. 

Any hatchery can rent a published agent or data from a harvester. Signing this transaction will withdraw $quantity * price$ domain tokens from the sender, where $price$ is the specific cost of the agent or data to which $UUID$ refers. The tokens are sent to the balance of the hatchery that created the agent or data. An additional $rentFee$ is withdrawn to restrict potential transaction spam, which is sent to the next tournament reward. Afterwards, the buying hatchery has to establish off-chain contact with the receiving hatchery and agree upon a delivery method, which is domain-specific. 

The transaction is valid if $quantity \geq 1$, the signer has enough balance to pay for the fees, $UUID$ exists, and a price for it has already been published through publish\_agent\_price or \mathbreak publish\_data\_price.

If $UUID$ refers to an agent whose payment scheme is to sell the algorithm directly, the transaction is invalid if $quantity \neq 1$.





\section{Attack resilience}
\label{attack-resilience}

In this section, we describe how the specifics of the ScyNet transaction protocol build resilience against the arbitrary failure of any network node and role.



\subsection{Underlying blockchain security}

The Tendermint framework allows for the synchronous processing of transactions that propagate through the network in a deterministic manner. There is no disparity in the system, meaning that replay attacks are not possible. Because of the voting mechanism for consensus, if one party obtains $\geq \frac{1}{3}$ of the network's consensus power, it can stop block verification. The system can be arbitrarily modified with $\geq \frac{2}{3}$ of the consensus power.

Additionally, the transaction signing makes impersonation is not possible without access to a node's private key.
%replay attacks, all handled by the fact that we're on a blockcain. byzantium tolerance (sign 2/3 of network block before happen)

\subsection{Transaction spam}

As discussed in the description of the transactions, every transaction type that does not require a fee has constraints on its usage for a time period. Sending a transaction outside of these limits will invalidate it and it will not be propagated through the network. Transactions with fees have monetary incentives against this behavior. This ensures protection against Denial-of-Service transaction attacks. 

\subsection{Agent signal copying}

A miner may be tempted to copy a rival's agent signals during a tournament and submit them as his own. However, all agent signals are submitted encrypted. The decryption key is revealed after the deadline for submission of a specific signal, protecting against copying.

A miner may instead copy all submitted ciphertexts of a rival and then copy the decryption key. However, when submitting a signal, the miner is required to encrypt both the signal and his public key, signing the package with his private key. This means that while cyphertext copying is possible, after the decryption key is revealed, so will be the true author.

\subsection{Service failure}

If a client has paid a miner or a harvester to utilize its agent or data, the providing node can theoretically deny access to the service, as it is not part of the blockchain consensus. However, as nodes on the network are usually anonymous, the provider has no financial incentive to behave that way.

\subsection{Agent submission failure}
%maybe not be so harsh for sending a decryption key later?

A miner may submit an agent for participation in a tournament and then fail to send a required timed agent signal or decryption key. In this case, the miner will be disqualified. If all miners in a tournament are disqualified, the tournament is still considered successful.

\subsection{Challenger failure}

In dataset domains, failing to send a dataset or an output decryption key by the deadlines will disqualify that challenger. This includes sending too large, wrongfully formatted, wrongfully encrypted, wrongfully hashed, or otherwise corrupt dataset.

Submitting a valid dataset with incorrect outputs is possible, as there is no way to differentiate between an inaccurate agent and bad testing data. The challenger can also secretly provide the unencrypted correct outputs to a competing miner, giving him an unfair advantage. Because the performance of an agent is his average performance over all challenger datasets, the intent is to minimize the impact of a malicious challenger by requiring a specific quantity of challengers as per Section \ref{challenger-actions}. Nevertheless, a theoretical large amount of malicious challengers can adversely impact the ranking reliability. 


\section{Off-chain node functionality}
\label{node-functionality}

Other than obeying the transaction protocol and defining the domain parameters, all nodes in a domain network must agree on the specifics of the problem in question. This includes defining the data format of the signals, harvester streams, and datasets, the method of evaluation of agent performance and any required external data, and the method of dataset generation for challengers (where applicable). Additionally, the miner software is responsible for executing and maintaining a NAS algorithm, as well as automatically selecting which neural networks produced by the NAS to submit for network verification as agents. 

In a realistic scenario, all of these actions will be performed through an open-source implementation of the ScyNet protocol for a specific domain. The intent is for the network to be autonomous and self-sustainable with no required human intervention in the lifecycle of its domains. 

==> content/predictor_content_en.tex <==
\section{Introduction}

Cryptocurrencies, the decentralized new ways of exchanging value, are gaining a lot of interest recently with the emergence of Bitcoin, Ethereum, and hundreds of other cryptoassets with total value that recently exceeded \$500 billion. Unlike the traditional markets, where all the data about the market and the trading itself are centralized and controlled by gatekeeper organizations, the cryptoasset markets are public, decentralized and transparent by definition.

%hypothesis
The new kind of data available on the blockchain can be analyzed together with standard market information in an attempt to predict future market movements.

%research goal
Our goal is to explore whether we can utilize the abundant blockchain data using modern Deep Learning techniques to estimate future facts about cryptoassets.

%say that blockchain is volatile and price data just won't cut it - comparison with world economical crisis
%Most forex and stock market predictions are based solely on previous price points. Similar prediction strategies, however, perform very poorly in the volatile cryptocurrency markets. To combat that we can analyze the public blockchain data, in addition to financial data, in an attempt to predict the future values.

%something about the framework?
%state how much is lost by volatility

%\subsection{Project Goals}

In this paper, we are introducing a set of methodologies for the cryptocurrency prediction problem and demonstrate their performance on the Ethereum ($ETH$) cryptocurrency \cite{yellowpaper}. First, raw blockchain and financial data is collected (Secton \ref{data-sources}), which is used in different feature extraction algorithms (Section \ref{property-generation}). The features are compiled into a dataset using different modeling techniques (Section \ref{dataset-generation}). Custom neural architectures are trained, evaluated and compared on their predictive performance (Section \ref{networks} and \ref{experiments}).

%We have concluded that the Ethereum blockchain ($ETH$) \cite{yellowpaper} is probably the most difficult to predict, due to its large and versatile user base. Some of its use cases include financial transactions, secure voting, autonomous organizations, company management, freedom of speech networks, online games, crowdfunding, speculation, and more. This stochastic environment will be the best to show the true performance of our prediction strategies, which can later be migrated to less noisy blockchains, like Bitcoin.

\subsection{Related work}

Projects about cryptoasset market predictions have emerged in the past, including a paper by a Stanford University team \cite{stanford-predictions} and two more recent Github projects \cite{bitpredict} \cite{deep-learning-bitcoin}. All of them focus primarily on Bitcoin price estimations, do not explore the rich publicly available blockchain data in depth, and do not use or have not disclosed sophisticated deep learning techniques for their estimations.

\input{content/common_content.tex}


\section{Generated datasets}
\label{generated-datasets}

The experiment setup includes a number dataset configurations. The interval of the datasets is from 2017-03-01 to 2017-11-01. This range contains the largest fluctuations in Ethereum's history, the widespread media hoax about Ethereum \cite{vitalik-death}, and the rise of ICOs \cite{ico}.

%we don't include any stateful LSTM experiments. No need to specify warmup dataset
Each complete dataset is split on $train$ and $test$ datasets.
%The first month of the range is reserved for the $warmup$ dataset. This part is only utilized in our stateful LSTM experiments and is used to initialize the network state before training or evaluation.
The first 7 months of the range build the $train$ dataset, on the basis of which the neural network is trained. The last month is utilized by the $test$ dataset, used for evaluation of the already trained network. 

% !!! I don't like how we refer to datasets here as complete, but as a matter of fact, they're not (wn, Norm & target are specified later).

The dataset configurations are defined in Table \ref{dataset_table}. Window size ($wn$), prediction target and the normalization ($Norm$) are specified later in the experiments. As datasets $1$ to $4$ do not include blockchain data, they are used as a baseline for comparison.

%multiple prediction targets?
\begin{table}[h]
\centering
\caption{The dataset definitions} \label{dataset_table}
\begin{tabular}{lp{6.0cm}r}
setN & Properties in dataset & Model \\\hline
1 & volumeFrom, volumeTo & matrix\\
2 & volumeFrom\_rel, volumeTo\_rel & matrix\\
3 & highPrice, volumeFrom, volumeTo & matrix\\
4 & highPrice\_rel, volumeFrom\_rel, volumeTo\_rel & matrix\\
5 & accountBalanceDistribution & matrix\\
6 & balanceLastSeenDistribution & stacked\\
7 & contractBalanceLastSeenDistribution & stacked\\
8 & balanceLastSeenDistribution, contractBalanceLastSeenDistribution, contractVolumeInERC20Distribution, accountBalanceDistribution & stacked\\
\end{tabular}

\end{table}

\texcomment{
\section{The genetic engine}
\label{genetic-framework}

Deep models usually have hundreds of hyper- and meta-parameters regarding the neural architecture, training parameters and dataset configuration that have to be individually tuned. The address space for possible configurations is too large compared to what we are able to optimize by hand. Our prediction framework allows for automatic tuning of some hyper-parameters by repetitive training, evaluation and respective parameter adjustments. This technique has been applied to our experiments. To automate the process further, we have chosen to create a genetic engine that aims to automate neural architecture search, hyper-parameter and dataset configuration by evolving agent machine learning models to accomplish a given predictive task.

An agent represents a deep network with its training parameters. An agent is created from a genome, consisting of a set of chromosomes. Each chromosome represents an array of integers with length based on the chromosome type. Example types include input data configuration, training parameters and a deep network layer with its their parameters (ex. $Conv2d$, $LSTM$). We have created a $JSON$ specification that allows the notion of any deep network configuration, and a converter that creates said $JSON$ from a genome. The output $JSON$ is passed to a parser that creates and returns the deep model, ready for training. 

\begin{figure}
\centering\includegraphics[width=\graphwidth]{assets/genetic_engine}\hfill
\caption{The structure of the genetic engine}
\label{genetic-framework-scheme}
\end{figure}

Please refer to Figure \ref{genetic-framework-scheme}. Initially, a population of $n$ individuals (genomes) is created with random chromosomes. Most chromosome values have limits (ex. the size of a deep layer cannot be a negative value). Each individual is passed through an initial check that modifies the chromosomes to be within all limits. Afterwards, the individuals are converted to our $JSON$ spec and parsed to deep models. Should the parsing stage fail (ex. an invalid combination of layers), the individual is killed. Reinforcement learning agents are created from these models and trained to emit signals of ``buy'' and ``sell'' for trading.
The properties included in the dataset of an individual are denoted in its genome. After training, each agent is evaluated and ranked with a fitness score based on their trading performance on a test dataset.

A set of new individuals is created via random binary mutations in the chromosome values, random chromosome addition/removal, Two-point crossover \cite{twopoint-crossover} and Uniform crossover \cite{uniform-crossover} from two parents, which are selected via Fitness proportionate selection and Tournament selection. The top $x\%$ of performing individuals are not mutated, while the worst ones are removed to keep the population number stable. The resulting set of individual's genomes are converted to $JSON$ and an agent is created for each one, which is trained afterwards. This algorithm is repeated until individuals with desirable performance are found.

The genetic engine is still under development and the following results and neural architectures do not take advantage of it yet.
\if\showlinks1
The engine is open source and available under \href{https://github.com/obecto/gattakka}{the following address: https://github.com/obecto/gattakka}
\fi
}

\section{Neural Network architectures}
\label{networks}

The experimental setup includes a Long Short-Term Memory (LSTM) \cite{LSTM} and a Convolutional (CNN) \cite{cnn} models. Their network architectures are described in Figure \ref{models}. 

The LSTM model, trained with datasets 1 to 4, is used as a baseline for comparison of the blockchain data approach. 

\begin{figure}[h]
\centering
\includegraphics[width=1.05\graphwidth]{assets/architectures_short_nodnn}
\caption{The architecture of the LSTM and Convoluitonal models respectively}
\label{models}
\end{figure}

\section{Experiments}
\label{experiments}

We have performed hundreds of experiments with different dataset configurations and neural architectures. Out of those, the best ones are selected and grouped per prediction target.

The performance measurements are taken after inverse normalizing the network output and are therefore normalization independent. All measurements besides $sign$ rely on the distance between the curves for prediction and actual values and are therefore directly incomparable between experiments with different targets. 

The experimentally selected optimal training parameters include batch size of $16$, $10^{-5}$ learning rate, and training via the Adam optimizer \cite{adam}. All networks are trained with these parameters.

\subsection{Predicting value ($highPrice$)}
\label{highPrice_exp}

\begin{table}[h]
\centering

\caption{\label{highPrice_table}Results for target $highPrice$.}
\begin{tabular}{lrrrrrrr}
$N$ & $setN$ & $win$ & $Norm$ & $Netw$ & $RMSE$ & $R^2$ & $sign$ \\\hline
%matrix-volumeFrom_rel,volumeTo_rel-highPrice-pixel-24w.pickle.pickle
1 & 2 & 24 & image & LSTM & 90.4185 & 0.9131 & 0.5258\\
%matrix-highPrice,volumeFrom,volumeTo-highPrice-property-8w.pickle.pickle
2 & 3 & 8 & prop & LSTM & 5.1060 & 0.9997 & 0.5095\\
%matrix-accountBalanceDistribution-highPrice-pixel-24w.pickle.pickle
3 & 5 & 24 & image & LSTM & 21.9306 & 0.9948 & 0.5054\\
%stacked-balanceLastSeenDistribution_cpp_log2-highPrice-pixel-104w.pickle.pickle
4 & 6 & 104 & image & CNN & 16.2167 & 0.9972 & 0.5115\\
%stacked-balanceLastSeenDistribution_cpp_log2-highPrice-pixel-8w.pickle.pickle
5 & 6 & 8 & image & CNN & 21.2845 & 0.9951 & 0.5033\\
%stacked-contractBalanceLastSeenDistribution_log2_v2-highPrice-property-104w.pickle.pickle
6 & 7 & 104 & prop & CNN & 83.1030 & 0.9265 & 0.5290\\
%stacked-contractBalanceLastSeenDistribution_log2_v2-highPrice-property-24w.pickle.pickle
7 & 7 & 24 & prop & CNN & 82.2199 & 0.9280 & 0.5367\\
\end{tabular}
\caption*{The shown measurements are the best ones from all training epochs.}
\end{table}

While the error scores on experiment $2$ seem impressive, the network cheats by returning the inputted previous price data, instead of making an actual prediction. Experiment $1$ does not input such information and forces the network to find an accurate solution. This can be seen in Figure \ref{1_2_highPrice}. In order to avoid such scenarios, the input data in all CNN experiments omits previous prices.

\begin{figure}[h]
\centering
\includegraphics[width=\graphwidth]{assets/1_highPrice}\\
\includegraphics[width=\graphwidth]{assets/2_highPrice}
\caption{$highPrice$: The test results of exp $2$ (bottom) and exp $1$ (top). We observe how exp $2$ achieves high accuracies by copying the previous price as a prediction and the result of omitting that data.}
\label{1_2_highPrice}
\end{figure}

Exp $3$ utilizes blockchain data and reaches an error reduction of 4 times compared to that of exp $1$. Despite not using any market data, the network is able to predict multiple major market movements (Figure \ref{3_highPrice}).

\begin{figure}[h]
\centering
\includegraphics[width=\graphwidth]{assets/3_highPrice_big}
\caption{$highPrice$: The test results of exp $3$. On multiple occasions, we observe valid reactions to major market movements.}
\label{3_highPrice}
\end{figure}

Exp $4$ includes more valuable blockchain data and combined with CNN results in the lowest error scores for this target (26\% lower than that of exp $3$).

The high errors on experiments $6$ and $7$ may indicate that $prop$ normalization is not suitable for distributions.

\subsection{Predicting relative value ($highPrice\_rel$)}

\begin{table}[h]
\centering
\caption{\label{highPrice_rel_table}Results for target $highPrice\_rel$.}
\begin{tabular}{lrrrrrrr}
$N$ & $setN$ & $win$ & $Norm$ & $Netw$ & $RMSE$ & $R^2$ & $sign$ \\\hline
%matrix-volumeFrom,volumeTo-highPrice_rel-property-104w.pickle.pickle
1 & 1 & 104 & prop & CNN & 2.3652 & -0.0031 & 0.5502\\
%matrix-highPrice_rel,volumeFrom_rel,volumeTo_rel-highPrice_rel-pixel-104w.pickle.pickle
2 & 4 & 104 & image & CNN & 2.3019 & 0.0498 & 0.4932\\
%stacked-contractBalanceLastSeenDistribution_log2_v2-highPrice_rel-pixel-24w.pickle.pickle
3 & 7 & 24 & image & CNN & 2.2825 & 0.0513 & 0.5340\\
%stacked-balanceLastSeenDistribution_cpp_log2,contractBalanceLastSeenDistribution_log2_v2,contractVolumeInERC20Distribution_log2_v2_stateless,accountBalanceDistribution-highPrice_rel-pixel-8w.pickle.pickle
4 & 8 & 8 & image & CNN & 2.2878 & 0.0461 & 0.5512\\
%stacked-balanceLastSeenDistribution_cpp_log2,contractBalanceLastSeenDistribution_log2_v2,contractVolumeInERC20Distribution_log2_v2_stateless,accountBalanceDistribution-highPrice_rel-property-104w.pickle.pickle
5 & 8 & 104 & prop & CNN & 9.1956 & -14.2060 & 0.5466\\
\end{tabular}
\end{table}

Because the next relative change, as a value, is too different from the last relative change, a network cannot increase its score without predicting accurately. This explains the small error difference between exp $1$ (volume data) and $2$ (price \& volume data).

Experiment $4$ utilizes 4 blockchain distributions and results in the lowest error and highest sign accuracy. However, when observing the prediction plot (Figure \ref{4_highPrice_rel}), the network is seen as less confident in its predictions. This may be mitigated with further network architecture and hyperparameter optimization.
% IS THIS LAST SENTENCE FOR HERE?

\begin{figure}[h]
\centering
\includegraphics[width=\graphwidth]{assets/4_highPrice_rel_big}
\caption{$highPrice\_rel$: The test results of exp $4$. The small $\sigma$ of the predictions suggests lower prediction confidence.}
\label{4_highPrice_rel}
\end{figure}


\subsection{Predicting user growth ($uniqueAccounts\_rel$)}

\begin{table}[H]
\centering
\caption{\label{uniqueAccounts_rel_table}Results for target $uniqueAccounts\_rel$.}
\begin{tabular}{lrrrrrr}
$N$ & $setN$ & $win$ & $Norm$ & $Network$ & $RMSE$ & $R^2$ \\\hline
%matrix-volumeFrom_rel,volumeTo_rel-uniqueAccounts_rel-property-104w.pickle.pickle
1 & 2 & 104 & prop & LSTM & 1139.972426 & 0.737456\\
%matrix-volumexFrom,volumeTo-uniqueAccounts_rel-property-104w.pickle.pickle
2 & 1 & 104 & prop & LSTM & 718.971374 & 0.895567\\
%stacked-contractBalanceLastSeenDistribution_log2_v2-uniqueAccounts_rel-pixel-8w.pickle.pickle
3 & 7 & 8 & image & CNN & 812.303885 & 0.864637\\
%stacked-balanceLastSeenDistribution_cpp_log2-uniqueAccounts_rel-pixel-24w.pickle.pickle
4 & 6 & 24 & image & CNN & 639.336022 & 0.916289\\
%stacked-balanceLastSeenDistribution_cpp_log2,contractBalanceLastSeenDistribution_log2_v2,contractVolumeInERC20Distribution_log2_v2_stateless,accountBalanceDistribution-uniqueAccounts_rel-pixel-8w.pickle.pickle
5 & 8 & 8 & image & CNN & 622.716696 & 0.920449\\


\end{tabular}
\end{table}

This set of experiments aims to demonstrate how blockchain data can be used to predict other facts about the blockchain, like how the amount of unique users will grow.

Sign accuracy is irrelevant in this case, as the number of\\ $uniqueAccounts$ always increases.

When predicting blockchain facts, it is not a surprise that the experiments with market data ($1$ and $2$) result in the lowest accuracies. Experiment $5$ (Figure \ref{5_uniqueAccounts_rel}) yields impressive results in all measurements, which is likely due to the 4 distributions in its dataset.

\begin{figure}[H]
\centering
\includegraphics[width=\graphwidth]{assets/5_uniqueAccounts_rel_big}
\vspace{-0em}
\caption{$uniqueAccounts\_rel$: The test results of exp $5$. The prediction curve follows the actual values relatively accurately.}
\label{5_uniqueAccounts_rel}
\end{figure}


\section{Results}

Through the experiments, we have observed the problem from different angles, by training different networks, dataset configurations, and evaluation metrics.

The results have shown that Ethereum is too volatile to be predicted based solely on market data.

The best overall results are achieved using the proposed blockchain analysis approach, confirming our initial hypothesis that this kind of data can assist predictions. The approach has demonstrated effective $4$ times reduction in error scores compared to only trade volume data. With the proposed Convolutional architecture, spatial account distributions, image normalization, and spatial dataset modeling, the error was additionally reduced by 26\%. Training times were also reduced by a factor of 10. 

Basic blockchain properties (as defined in Table \ref{properties}) have demonstrated to be inefficient for the predictive task. These findings are consistent with the lower hourly prediction scores on the Bitcoin trading research by the Stanford research group \cite{stanford-predictions}.

The spatial distributions have been consistently linked to the highest accuracy results, as they are able to analyze the blockchain raw data in more depth than other approaches.

The overall best dataset found combines all 4 of the spatial distributions (Number $8$ in Table \ref{dataset_table}), modeled by the Stacked layers model (Section \ref{stacked-model}). The best found prediction target is relative high price, which forces the models to find the best possible predictive strategy. 

The overall most accurate neural network is the proposed Convolutional model. Its ability to extract spatial meaning from the data likely contributes to its success in the distributions.

%UNNEEDED
%We recommend batch size of 16, which provides balance between training times and network generalization. There are methods to increase accuracy with large batches \cite{accurate-large-batch}, but a smaller batch is always better in terms of generalization.

The best blockchain approach includes many parameters that have to be further explored before we can state the extent to which blockchain data can assist predictions.

\if\showtech{1}

\section{Technical implementation}

For our experiment, we have created and documented a robust framework which can be used as a foundation for the development and training of models that predict facts about any blockchain and based on any data. All the referenced in this paper properties, dataset models, normalization strategies and the aforementioned techniques are all included in the source code provided with the open source framework. 

The framework is split into multiple tools for managing data download and storage, property generation, dataset generation, and neural network training and evaluation:

\begin{itemize}
\item \textbf{Dataset extraction module}: responsible for connection to data providers (like the ones discussed in Section \ref{data-sources}), download, validation of integrity, and storage of the raw data.

\item \textbf{Data storate module}: reads and post-processes the raw data by filtering out unimportant for our research data and saving the rest as a time series in a database. For fast retrieval by date interval, the data is split by a chunking algorithm.

\item \textbf{Property generation module}: generates and stores time series of property values (discussed in Section \ref{property-generation}) by utilizing the raw time series data.

\item \textbf{Dataset generation module}: normalizes the property values and applies a chosen dataset model to generate a dataset (the process is described in Section \ref{dataset-generation}).

\item \textbf{Training and evaluation module}: trains and evaluates a chosen neural architecture on a specified dataset (our proposed architectures are in Section \ref{networks} and our error measures are described in Section \ref{measures}).
\end{itemize}


\subsection{Automated tests}

We have implemented unit and integration tests for all of our tools, where applicable. This is done to ensure that the dataset generated by those tools is always with the expected and true values.


\section{Technologies}

\begin{enumerate}
\item \textbf{JavaScript} is used for the data extraction module;
\item \textbf{Web3 API} allows the extraction of blockchain data from a local running Ethereum node;
\item \textbf{Node.js} creates connections to other APIs for the rest of our raw data;
\item \textbf{Python} is used for all other modules;
\item \textbf{Pandas} provides high-performance data structures and data analysis tools for Python;
\item \textbf{MongoDB} is the database we use to store our data throughout all stages of data processing;
\item \textbf{Arctic} is a high performance datastore for numeric and time-series data used in hedge funds;
\item \textbf{Tensorflow} is the Deep Learning library most commonly used in Deep Learning research and development;
\item \textbf{Keras} is a frontend framework for a backend (like Tensorflow) that allows quick development of neural network architectures;
\item \textbf{Scala} is used in the core of the genetic framework;
\item \textbf{Akka} is a framework for the actor model, implemented in the genetic framework, allowing scaling of agent optimization tasks over multiple computing nodes simultaneously.
\end{enumerate}

\fi

\if\showlinks1
\section{Cryptocurrency prediction framework}

The technical implementation of the data processing, dataset generation and neural network evaluation processes is developed into an open source Cryptocurrency prediction framework. The framework allows for the prediction of a chosen cryptocurrency on the basis of user-defined property extraction and neural algorithms. \href{https://github.com/Zvezdin/blockchain-predictor}{The framework can be accessed at: https://github.com/Zvezdin/blockchain-predictor}

The repository includes the necessary technical documentation for the reproduction or improvement of our experimental results.

All trained model weights, detailed training histories, and performance visualizations, are available \href{https://goo.gl/uBQn4p}{here: https://goo.gl/uBQn4p}.

\texcomment{
\section{Future work}

Throughout the research, we have evaluated not only a number of Deep Learning models but we have also built a reusable framework for data gathering, processing and storage of blockchain and market data. Once we had this framework, most of our actual research work was reduced to trying different network architectures and meta-parameters. While this process alone was challenging and demanding of both deep knowledge and creative thinking, we are excited by the possibilities to experiment with automating it. 

Two recent publications by Google Research \cite{automl-genetic} \cite{automl-rl} show that given enough computing power, we can create a ``controller'' algorithm which produces model designs for predicting the CIFAR10 dataset \cite{cifar-10}, with performance on par with state-of-art models designed by humans. The process is called neural architecture search (NAS). The authors emphasize the enormous computational power required for achieving these results which was in order of $10^{20}$ computation. For comparison, most estimations about the computational power of the human brain are for between petascale ($10^{15}$) and exascale ($10^{18}$) operations per second \cite{brain-processing-power}.

We are interested in exploring NAS methodologies in order to find the most optimal neural configuration for blockchain data analysis.

Furthermore, we hope to develop a scalable decentralized architecture which allows remote nodes to provide computing power to ``controller'' algorithms for evaluating individual Deep Learning models. In such a system, Ethereum smart-contracts can be utilized to implement a decentralized marketplace for neural network model training and optimization. 

Blockchain mining, which consumes enormous amounts of electrical power \cite{electricity-for-mining}, might soon become obsolete due to the adoption of more efficient consensus algorithms like Proof-of-Stake. This presents an unique opportunity to utilize the abundant GPU mining resources for more reasonable work, like training Deep Learning models.
}

%NEEDED?
%We are excited to work towards our new research goal during 2019, since this year might present a unique opportunity to build the first decentralized exascale supercomputer dedicated for training AI.


\section{Conclusion}

%NEEDED?
Blockchain technology enables a new class of tradable cryptotoken assets, thus creating new kinds of markets with numerous new use cases. Due to their decentralized and open nature, public blockchains provide an abundance of market-related data that has never been available before. Having every account balance and every transaction visible encourages us to seek a holistic view on the blockchain dynamics.

In the article, we have evaluated different Deep Learning methods at their ability to find patterns in the Ethereum blockchain data and provide estimations about future measurements of the blockchain assets, including their market price. To facilitate our experiments, we have implemented a data gathering, processing, and storing framework that enabled us to deal with the enormous amount of data on the blockchain (more than 1000GB) and efficiently produce datasets for training.

We have tested both Recurrent and Convolutional models with different data sets and prediction targets. The most interesting results came from our Convolutional models which were working on account distribution histograms with one, two, and three dimensions. These histograms serve as ``pictures'' of the blockchain in a certain period of time and when we observe
\if\showlinks1
a \href{https://youtu.be/Dwwnxn1j6AQ}{time-lapse video of such 2D histograms (https://youtu.be/Dwwnxn1j6AQ)},
\else
their historical values,
\fi we can clearly see patterns that correlate to major market moves. After experimenting with these novel blockchain data representations, we found that Convolutional Deep Learning models are capable of providing estimations for the ETH token price based solely on such histogram data. Still, we believe that better results can be achieved by further optimizations of the model architectures and meta-parameters.

Since the search space for such optimizations is enormous, we will be focusing on creating efficient Neural Architecture Search approaches that automate the search process. We will also be investigating different ways in utilizing independent GPU resources in the common goal of finding a more efficient neural network.


%TODO: Wait for kosta reply
%\section{Acknowledgements}

%We would like to thank HSSIMI for allowing us to start our research at the Summer Research School.


==> content/scynet_spec.tex <==
\newcommand{\mathbreak}{\\} %temporary workaround to math sections not receiving line breaks before them.

\section{Distributed NAS in a blockchain}
\label{scynet}

One possible way to counter this problem is to create an open environment where financially incentivised computing nodes can execute NAS algorithms and compete with each other in finding optimal neural solutions to a specific problem. 

This is the idea that lead us to the creation of a general framework and blockchain protocol for distributed creation of autonomous machine learning agents named ``ScyNet''. 

The following subsections provide a high-level overview of the protocol in question. The formal definition of the transaction protocol and node responsibilities is found in Appendix \ref{formal-scynet}. Explanation of the possible attacks a malicious actor can attempt, as well as how the system will handle these scenarios, is found in Appendix \ref{attack-resilience}.

\subsection{Main entities and roles}

A specific implementation of ScyNet for a chosen problem (for example, stock market predictions) represents a single blockchain network and is called a \textbf{Domain}. Every domain defines an unique utility token that is used to form consensus and incentivise participants. A node, member of a domain network, is called a \textbf{Hatchery}. Three types of hatcheries exist - harvesters, miners, and external clients. Harvester hatcheries interface the real world by selling data related to the domain problem. Miner hatcheries use that data to execute a NAS that creates machine learning \textbf{agents} as potential solutions to the problem. The network consensus verifies the performance of the agents and financially awards the best ones. Then, clients can explore the verified agents and utilize them for a specific subscription fee determined by the hatchery that produced them. 

For example, if we were to apply this protocol for the blockchain problem, we would create a domain for cryptoasset predictions. Harvesters can provide arbitrary blockchain or market analysis data and miners can purchase this data to train predictive agents. Client hatcheries can rent and use these predictive algorithms to trade their own portfolio.

\subsection{Tournament validation}

Tournaments are regularly scheduled ``competitions'' for the verification of new agents. They have a start date and a specific duration, after which the next tournament starts. Miner hatcheries have the right to submit one or more of their agents for verification by paying a submission fee before the start of the next tournament. 

How a tournament can cryptographically prove an agent's performance depends on the type of machine learning problem being solved in the domain. The first type represents real-time predictions, such as stock market trading or weather forecasts. These predictions are made at the same time in a consistent schedule, known as real-time ticks. In this scenario, the competing miners are requested to provide real-time predictions from their agents for every tick during the tournament. Afterwards, every node in the network compares these predictions to the actual values to form consensus on a ranking of the participating agents and their respective performance.

The other type of problems are dataset input-output problems, such as self-driving algorithms or speech recognition. In this case, the network consensus randomly selects multiple nodes that are labeled as \textbf{challengers}. Every such node is responsible to provide a dataset with which to challenge the competing agents to resolve it. Depending on the problem, this can be either algorithmically generated, or retrieved from a reliable source. The miners evaluate the dataset and publish the outputs of their agents. After tournament closure, the network compares the agent outputs to the expected ones and forms consensus on an agent ranking.

The submission fees collected before a tournament comprise the tournament award, which is used to award the top performing agents and the selected challengers, if applicable.

At no single point do the miners reveal the mechanisms behind their agents, allowing for a significant flexibility in how these agents are created.

\subsection{Agent utilization}

Miners with verified agents have the right to set a price and allow others to ``rent'' their agents. For real-time problems, this means paying a subscription to receive a specific agent's real-time predictions. In dataset problems, the clients privately send a specific input data that they want the agent to resolve and then receive its output, paying a fee for every input they submit. A miner that does not want to sustain an agent can also directly sell the model behind it. The fees are received directly by the respective seller miners as an additional reward for having created useful agents.

Other than being sold to external clients, agent outputs (signals) can also be bought by miners that include them in the input of their own agents. This act of chaining agents also means that there can be ``aggregator'' agents that receive signals from many other agents and produce a more informed signal on their own.

%For example, in one simplified domain, we can have a harvester hatchery that provides stock market data flow and a miner hatchery that purchases this data to produce predictive algorithms for the stock market. Finally, a client hathery may rent and use these predictive algorithms to trade its own portfolio.





==> front/abstract_bg.tex <==
%Пазарите на криптовалутите надвишават 500 милиарда долара маркетингова капитализация, като интересът към тях расте експоненциално последните месеци. Борсите за крипто-активи са обществени, децентрализирани и прозрачни по дефиниция и позволяват нов начин за обмен на стойност без посредник. Поради това тяхно свойство, криптовалутите често са непостоянни и нестабилни за използване. В нашето изследване, ние проучваме новия вид данни, налични в блокчейна на Ethereum, в усилия да създадем точна стратегия за прогноза на бъдещи факти чрез използване на дълбоки невронни мрежи. За нашия експеримент ние създадохме и документирахме гъвкава рамка, която позволява да се предскаже всяка черта на всяка криптовалута на базата на всякакви данни.

В нашето проучване ние изследваме как съвременните техники за дълбоки невронни мрежи могат да бъдат приложени за прогнозиране на бъдещи факти за блокчейна на Ethereum. По-конкретно, ние се интересуваме дали публичните данни в блокчейна, като броя на транзакциите и дистрибуцията на балансите, могат да бъдат използвани за прогнозиране на други мерки, като броя на създадените нови акаунти и пазарната цена на валутата.

Сред поредица от експерименти с блокчейн данни, ние постигнахме 330\% по-ниска грешка спрямо LSTM решение работещо само върху пазарните данни. Ние намалихме грешката с допълнителни 35\%, използвайки дистрибуции на балансите, пространствено моделиране на данните и конволюционна невронна ахритектура.

Освен това, разработихме и преизползваема рамка, позволяваща извличане, обработка и съхранение на блокчейн данни, както и извършване на експерименти с дълбоки невронни мрежи върху тях. Нашите бъдещи планове са насочени към развиване на контролер невронни мрежи, които автоматично генерират невронно-мрежови архитектури и оптимизират техните хиперпараметри постигане на по-добри резултати в дадена задача. За тази цел е възможно да се използва голямото количество GPU мощност в Ethereum мрежата, което скоро ще остане ненужно поради приемането на Proof-Of-Stake алгоритъма за консенсус. Ние вярваме, че 2018 година представлява уникална възможност за постигане на децентрализиран суперкомпютър, отдаден на създаването на изкуствен интелект.

%Борсите за крипто-активи са обществени, децентрализирани и прозрачни по дефиниция. В нашето изследване, ние проучваме новия вид данни, налични в блокчейна на Ethereum, в усилия да създадем точна стратегия за прогноза чрез използване на дълбоки невронни мрежи. Събираме данни си от няколко източника и извличаме от тях най-важните и стойностни моменти (свойства). Освен основни свойства, изследваме и различни методи за създаване на цялостни картини на състоянието на мрежата, като генерираме множество стойности, които са специално подредени във времето и пространството. Ние предлагаме няколко метода за моделиране на набор от данни, които подреждат стойностите на свойствата по различен начин в многомерно пространство. Изграждаме архитектури на невронни мрежи, базирани на основната дълбока мрежа, Long Short-Term Memory (LSTM) и конволюционна мрежа. Проведохме различни експерименти с различни набори от данни с всяка от тях. Понеже конволюционната мрежа е способна да извлича смисъл от пространствено свързани данни, тя е далеч по-точна от всеки друг модел, с който сме експериментирали. Поради високата си непостоянност, Ethereum се оказа изключително трудна за предсказване. Независимо от това, резултатите ни показват силна зависимост между данните за блокчейна и цените. Трябва да фокусираме повечето от усилията си върху усъвършенстването на качеството на нашия набор от данни, преди да се насочим към мрежовата архитектура. Установихме, че увеличаването на пространствената стойност в нашия набор от данни също увеличава точността на прогнозата.

%За нашия експеримент ние създадохме и документирахме гъвкава рамка, която позволява да се предскаже всяка криптовалута на базата на всякакви данни.

==> front/front_bg.tex <==
\selectlanguage{bulgarian}

%short: Прогнозиране на базата на блокчейн данни
\title{Прогнозиране на криптовалути на базата на публични блокчейн данни}
\author{Автор: Звездин Бесарабов \\ Национална природо-математическа гимназия \\ \href{mailto:me@zvezd.in}{me@zvezd.in} 
   \and Под ръководството на Тодор Колев \\ Председател на Комрад кооператива \\ \href{mailto:todor@comradecoop.com}{todor@comradecoop.com} }

\thispagestyle{fancy}

%\renewcommand\maketitlehooka{\null\mbox{}\vfill}
%\renewcommand\maketitlehookd{\vfill\null}

%\begin{titlingpage}
\maketitle
%\end{titlingpage}
%\newpage
\begin{abstract}

\input{front/abstract_bg.tex}

\end{abstract}

==> front/front_en.tex <==
\selectlanguage{english}

%short: Predictions based on blockchain data
\title{Estimating future facts about digital assets based on blockchain activity data}
\author{Author: Zvezdin Besarabov \\ National school of mathematics and natural sciences \\ \href{mailto:me@zvezd.in}{me@zvezd.in} 
   \and Under the guidance of Todor Kolev \\ Founder of the Obecto Cooperative \\ \href{mailto:todor@comradecoop.com}{todor@comradecoop.com} }

%\date{August 15, 2017}
\maketitle

\begin{abstract}

\input{front/abstract_en.tex}

\end{abstract}

==> front/front_hssimi.tex <==
\includepdf[pages={1}]{assets/UK18-title_page.pdf}

\newpage

\selectlanguage{bulgarian}

\begin{abstract}

\input{front/abstract_bg.tex}
\end{abstract}

\selectlanguage{english}

\begin{abstract}

\input{front/abstract_en.tex}

\end{abstract}

==> front/front_isef.tex <==
\selectlanguage{english}

\title{Predicting digital asset market based on blockchain activity data}
\author{Author: Zvezdin Besarabov \\ National School of Mathematics and Natural Sciences \\ \href{mailto:me@zvezd.in}{me@zvezd.in} 
   \and Supervisor: Todor Kolev \\ Chairman of the Comrade Cooperative \\ \href{mailto:todor@comradecoop.com}{todor@comradecoop.com} }

%\date{August 15, 2017}
\maketitle

\thispagestyle{fancy}

\fancyhead[c]{Intel International Science and Engineering Fair 2018}

\begin{abstract}

\input{front/abstract_en.tex}

\end{abstract}

==> front/gsf_abstract_en.tex <==
The vast availability of data and computing power allowed Deep Learning to thrive with applications in virtually every area. Creating efficient Deep Networks involves repetitive manual tuning of network topologies and hyperparameters. This human intervention significantly impacts development time.

Recent publications propose various Neural Architecture Search algorithms that automate this process. This motivated us to investigate how we could create or improve the theoretical background of such an algorithm and expand its application in the field.

In this research we introduce and evaluate two NAS approaches: a genetic algorithm and a modified NAS with network morphism and bayesian optimization. The algorithms are scored based on their ability to create solutions for the cryptocurrency prediction problem.

A baseline experiment with manually configured Neural Networks reached a predictive accuracy of 55\%. Focusing on short-term adaptation and using the modified NAS algorithm, an automatically generated Neural Network reached 78\% accuracy. The genetic algorithm also delivered impressive results and produced a network that reached $1.8$ times investment returns in simulated $ETH$ trading for a period of 6 months. 

While exploring these NAS approaches we have noted various shortcomings of the algorithms that are yet to be explored and may yield better results.

==> front/nas_abstract_bg.tex <==
Блокчейн технологията демонстрира голям потенциал в своето изграждане като свързващо звено между всяка индустрия и пазар, позволявайки децентрализиран и сигурен обмен стойност и свързвайки цивилизацията както никога преди.

Типичният подход при валутни прогнози е основан върху пазарен анализ с LSTM невронна мрежа. Блокчейн технологиите, обаче, ни дават достъп до големи количества публична информация, примерно като изпълнените трансфери и разпределението на балансите по потребителите. Ние разучаваме дали анализирането на тази информация с дълбоко машинно самообучение резултира в по-високи прогнозни точности спрямо типичния подход.

Най-добрата публикация до момента относно темата за ефективно търсене на невронно-мрежови архитектури с мрежов морфизъм ни мотивира да разгледаме как може да подобрим теоретичната основа на този алгоритъм и да разширим неговото приложение в сферата.

Първичните експерименти на този алгоритъм с блокчейн-базиран датасет разкриват обещаващи прогнозни точности и ни стимулират да доразвием планираните подобрения по алгоритъма, както и за неговото приложение в проблема за прогнози на крипто борсата.

==> front/nas_abstract_en.tex <==
Creating efficient deep neural networks involves repetitive manual optimization of the topology and the hyperparameters. This human intervention significantly inhibits the process.

Recent publications propose various Neural Architecture Search (NAS) algorithms that automate this work. We have applied a customized NAS algorithm with network morphism and Bayesian optimization to the problem of cryptocurrency predictions, where it achieved results on par with our best manually designed models. This is consistent with the findings of other teams, while several known experiments suggest that given enough computing power, NAS algorithms can surpass state-of-the-art neural network models designed by humans. 

In this paper, we propose a blockchain network protocol that incentivises independent computing nodes to run NAS algorithms and compete in finding better neural network models for a particular task. If implemented, such network can be an autonomous and self-improving source of machine learning models, significantly boosting and democratizing the access to AI capabilities for many industries.



%The vast availability of data and computing power allowed deep learning to thrive with applications in virtually every area. Creating efficient deep neural networks involves repetitive manual optimization of the topology and the hyperparameters. This human intervention significantly impacts development time.

%Last year, we developed manual neural networks for cryptoasset predictions. 

%Recent publications propose various Neural Architecture Search (NAS) algorithms that automate this process. More recent is a modified NAS with Network morphism and Bayesian optimization. After applying and optimizing the algorithm for cryptocurrency predictions, we noticed sharp accuracy scores (78\% with 70\% baseline) as compared to our experiments with manual tuning of neural networks  (55\% with 50\% baseline).


%As NAS results' accuracy is improving with more computing power being utilized, we desi

%Throughout our experiments we noticed that the NAS results' accuracy is improving as more computing power is utilized. This paper introduces a distributed blockchain protocol that incentivises independent computing nodes to run NAS algorithms and compete to find better neural network models for a particular task. 

%A network with this protocol can be implemented to 

%If a network with this protocol is implemented, it will be practically autonomous source of 

%Implementing this protocol in an operational blockchain network is important in providing access to the latest state of machine learning results, freely available for every entity to utilize and contribute to. Hence our next steps are providing a configurable blockchain node implementation, suitable for a larger variety of machine learning problems.



%This motivated us to investigate how can we create we could create or improve the theoretical background of such an algorithm and expand its application in the field.

%In this paper we introduce and evaluate two NAS approaches: a genetic algorithm and a modified NAS with network morphism and bayesian optimization. The algorithms are scored based on their ability to create solutions for the cryptocurrency prediction problem.

%A baseline experiment with manually configured Neural Networks reached a predictive accuracy of 55\%. Focusing on short-term adaptation and using the modified NAS algorithm, an automatically generated Neural Network reached 78\% accuracy. The genetic algorithm also delivered impressive results and produced a network that reached $1.8$ times investment returns in simulated $ETH$ trading for a period of 6 months. 

==> front/predictor_abstract_en.tex <==
%Predicting the future is impossible. Yet, the better estimation we have about the future, the more power we h	ave to make the most optimal decision in the present. 

Blockchain technology shows significant results and huge potential for serving as an interweaving fabric that goes through every industry and market, allowing decentralized and secure value exchange, thus connecting our civilization like never before.

The standard approach for asset value predictions is based on market analysis with an LSTM neural network. Blockchain technologies, however, give us access to vast amounts of public data, such as the executed transactions and the account balance distribution. We explore whether analyzing this data with modern Deep Leaning techniques results in higher accuracies than the standard approach.

%In our paper we explore how modern Deep Learning techniques can be applied to predict future facts about the Ethereum blockchain. Specifically, we are interested if blockchain's public raw data, such as the transaction count and the account balance distribution, can be used to predict other measures like the number of new accounts created and the market price per ETH token.

During a series of experiments on the Ethereum blockchain, we achieved $4$ times error reduction with blockchain data than an LSTM approach with trade volume data. By utilizing blockchain account distribution histograms, spatial dataset modeling, and a Convolutional architecture, the error was reduced further by 26\%.

The proposed methodologies are implemented in an open source cryptocurrency prediction framework, allowing them to be used in other analysis contexts.

%Moreover, we have developed a reusable framework providing data gathering, processing, and storing functionality for performing Deep Learning experiments over blockchain data.
%Our future plans are towards automating neural network architecture and meta-parameter optimization tasks through training controller Machine Learning models on these tasks. Since the Ethereum network already utilizes a great amount of GPU processing power, which might become obsolete due to the adoption of a Proof-of-Stake algorithm, we believe that 2018 presents a unique opportunity for achieving an exascale decentralized supercomputer, dedicated to training AI.

%----------------

%The crypto-asset markets are public, decentralized and transparent by definition. In our research, we explore the new kind of data available on the Ethereum blockchain in efforts to create an accurate prediction strategy using deep neural networks. We gather our data from multiple sources and extract the most important data points (properties) from it. Other than basic properties, we explore different methods to create complete network state snapshots by generating multiple values that are specifically ordered in time and space. We have proposed multiple methods to model a dataset by aligning the property values differently in multidimensional space. We have built neural network architectures that are based on basic deep, Long Short-Term Memory (LSTM) and Convolutional networks. We ran different experiments with each one of them and with different datasets. Because the convolutional network is able to extract meaning from spatially related data, it performed far superior than any other model we have tried. Due to its high volatility, Ethereum has proven difficult to predict. Despite that, our results have shown a strong correlation between blockchain and price data. We should focus most of our efforts in perfecting the quality of our dataset, before tweaking the network architecture. We have found that increasing the spatial value in our dataset also increases the prediction accuracy.

%For our experiment, we have created and documented a flexible framework that allows the prediction of any cryptocurrency on the base of any data.

